Player-AI Interaction: What Neural Network Games Reveal About AI as Play

The advent of artificial intelligence (AI) and machine learning (ML) bring human-AI interaction to the forefront of HCI research. This paper argues that games are an ideal domain for studying and experimenting with how humans interact with AI. Through a systematic survey of neural network games (n = 38), we identified the dominant interaction metaphors and AI interaction patterns in these games. In addition, we applied existing human-AI interaction guidelines to further shed light on player-AI interaction in the context of AI-infused systems. Our core finding is that AI as play can expand current notions of human-AI interaction, which are predominantly productivity-based. In particular, our work suggests that game and UX designers should consider flow to structure the learning curve of human-AI interaction, incorporate discovery-based learning to play around with the AI and observe the consequences, and offer users an invitation to play to explore new forms of human-AI interaction.

==> files.tex <==

Code rubric
https://docs.google.com/document/d/1pIPI9A-1il6fPOrFzIjEwwvB7IJWTbVf9GN89YyPmtc/edit?usp=sharing

Code spreadsheet
https://docs.google.com/spreadsheets/d/1sF3sO7bnCngIFI4WiyCn2zMfAjJFjvnYbkVwLmXgoHs/edit?usp=sharing


DATA:

Game list and description
https://docs.google.com/document/d/1KlfbAmSSodjXG5qwNOn5EIezSHgkaeirToa6hFZxfkw/edit?usp=sharing

Play session footage
https://drive.google.com/drive/folders/1vbRIV6NpsOfZp-0fmv0oSexiDB41L9qG?usp=sharing 

==> glossary.tex <==
\newacronym{ann}{NN}{Neural Network}
\newacronym{pcg}{PCG}{Procedural Content Generation}
\newacronym{hci}{HCI}{Human-Computer Interaction}
\newacronym{gar}{GAR}{Galactic Arms Race}
\newacronym{dm}{DM}{Dungeon Master}
\newacronym{lm}{LM}{Language Model}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{npc}{NPC}{Non Playing Character}
\newacronym{dnn}{DNN}{Deep Neural Network}
\newacronym{rq}{RQ}{research question}

==> prev_submission/06_Discussion.tex <==
\section{Design Implications}
Through the specific case of NN games, we have demonstrated the richness of player-AI interaction as a research topic. In this section, we intend to situate player AI interaction in the broader context of related research areas. We then distill the design implications of our study for the games and for UX/HCI. 

\subsection{Why player AI interaction}
The study of players, game design, and game technology (here we focus on AI) are three main pillars in games research (Figure \ref{fig:researchAreas_vennDiagram}). At the intersection of Games and AI, there is a well-established research community of game AI. Combining the study of player with game design, there is the research area of player experience. However, the intersection between players and AI has so far been relatively under-explored. Until recently, real players are typically only brought in at the end of game AI research as the means to evaluate the effectiveness of the algorithms. Curving out the topic of player AI interaction will fill in the gap. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/reserchareas_venn.pdf}
    \caption{Research areas around games.}
    \label{fig:researchAreas_vennDiagram}
\end{figure}



%With the rapid advancement of AI during the last couple of decades, one might expect the NN to takeover existing design tasks currently carried out by other algorithms or humans.
%From our observations, the NN was indeed a replacement of an existing algorithm—-for example, determining fight or flight behavior for enemy units in \emph{Supreme Commander 2} \citeL{rabin2015game}. Without an extensive study of the behavior of this NN, one cannot argue whether this application of NN was justified or could be replaced by more straightforward approaches.

% In most of the studied cases, it is instead the situation that NN and traditional game mechanics co-exists. This is particularly clear in the cases of \emph{NN as designer}. For instance, in \emph{Galactic Arms Race} \citeL{hastings2009evolving}, a significant amount of traditional, manual, game design was still required; the NN was simply a novel game component that needed to be integrated with the game, and involved a delicate integration process. Similar cases can be made for \emph{Creatures} \citeL{grand1997creatures}, \emph{Petalz} \citeL{risi2015petalz}, \emph{How to Train your Snake} \citeL{snake}, amongst others. We observed the NN as more of an \emph{support} to the existing game mechanics rather than offering novel mechanics that we have not seen before.

% Generally speaking, NN are extremely flexible and work well for more complex applications that require many dimensions in player input and NN output. NN can be utilized in countless ways, and, if done correctly, can generate interesting solutions and gameplay experiences. Applying NN in the context of games allows for deeper experiences not previously possible. An example is \emph{AI Dungeon} \citeL{aidungeon}, which heavily relies on the generative properties of the NN. While the game utilizes existing core mechanics, the infinite creation of new, meaningful adventures is not feasible to be done beforehand by a game designer. As a result, the NN creates an endless experience that is unique each time for each player.
% In most of the studied cases, the advantage of applying NN comes from this ability to generate content or behaviors that can be used during gameplay, which we observed in \emph{AI Dungeon}, \emph{Galactic Arms Race}, and others. 

%what can the ai community take away from this?
%what are the design implications of human-ai interactions in nn games?
%How are these games different?
%what are the implications for game design?

\subsection{Implications for Games}
In addition to establishing games as a rich domain for human-AI interaction, our analyses contribute insights into how games can improve the interaction between players and AI.  Based on our findings from section \ref{sec:guide_results}, game designers interested in a complementary dynamic between the player and AI (NN as Teammate) would benefit from implementing guidelines such as G16 ``convey the consequences of user actions related to NN'' and G18 ``clear notifications of changes in NN capability.'' By providing players with a visualization of how their actions may impact the NN, players may be more equipped to better understand when to step in for the NN or when the NN should take over given the gameplay objective, thus fostering a more collaborative dynamic. Further, designers may also explore Guideline G17 ``provide global controls'' as a way to visualize what the system can do, as this may develop new interactions between players and AI.

%{\color{red} Add what game designers do based on our findings in section 5 when they design AI-based games? It will probably be something related to the guidelines.}

\subsection{Implications for UX and Human-AI Interaction}
For UX designers and HCI researchers interested in human-AI interaction, our key take-away is that reframing {\bf AI as play} offers a useful approach to improve existing UX design for AI-based applications and to expand our notions of what human-AI could be.

{\bf Use the concept of flow to structure the complexity of user interaction with the AI}. For most users, interaction with AI can be overwhelming, especially when they encounter unexpected output from the AI. One important lesson from our collection of games is that the concept of flow can be used to structure the difficulty level of the human-AI interaction. The psychological concept of flow~\cite{csikszentmihalyi1990flow} is widely adopted by game designers to engage the player. UX designers of AI-infused products can apply this concept so that the user's interaction with AI strikes the right balance between too challenging (thus overwhelming) and too easy (thus boring). 

{\bf Incorporate enhanced discovery-based learning}. Many games in our analysis, especially simulation games, offer discovery-based learning~\cite{alfieri2011does} with mixed success. Since players come with different background knowledge and needs, explicit instruction for AI is challenging to design. Discovery-based learning offers the players the opportunity to play around with the NN at their own pace and observe the consequences of their actions on the NN and the game world. However, most NN games in our dataset offered very little scaffold, making it difficult for players without a technical background to succeed. We suggest UX designers use enhanced discovery-based learning and provide feedback, worked examples, scaffolding, and elicited explanations to further assist their users. 


{\bf Extend the invitation to play.} Finally, for researchers and designers who are interested in exploring new forms of human-AI interaction, we believe offering users an invitation to play can unleash their imagination and empower them to explore new ways to interact with even the same technology. As we can see from {\em Hey Robot!}, the magic circle of play turns the smart speaker user from the seeker of information to the provider. The voice assistant's inability to understand user command/intent is transformed from failure to perform to the source of fun. 


%These AI-infused products could benefit from flow if they maybe consider the current (get them what they need) and longer endeavor (what else will they need in the future)? But aren't some of these products doing this already? Hm...

%\begin{enumerate}
    
 %   \item Theme 1: Games are a good environment to study UX interactions.
    
%        - NN simulation games more often comply with the guidelines. They make the NN the main focus of the interaction. They provide 1) openness with global controls and 2) feedback with UI and behaviors. This combination leads to experimentation.
        
%        - In these games, they allow players to link their preference with the NN output. A dynamic that HCI can further investigate.
        
 %       - With experimentation comes with frequent failure. Failure is something that should not happen in UX. Games ar eunique in this sense to look at human-ai interactions in a safe environment. By something going wrong, the player is better equipped to understand the systems limitations through play. 
        
%        - We are still at an early stage, but we start seeing new interactions, such as NN as Teammate where both share an objective. However, more work is needed to explore in the context of human-ai complimentary dynamic.
        
%        - Human-AI complementarity dynamic can be something that can be studied through games. None of the games in our corpus lets the player know clearly about the NN limitations, however 48\% make the capabilities of the NN known to the player.
    
 %   \item Theme 2: We need more guidelines.
    
%        - The majority of the guidelines apply to teammate and apprentice interactions.
        
%        - When the UX is to strive for mastery or competence in NN as competitor, these guidelines would not be suitable. For example, knowing the limitations would lead to ruining the suspense or players to exploit these to win more easily. 
        
%        - When the UX is about control in NN as apprentice, puzzling about how to best guide or direct the NN becomes the challenge. Knowing the limitations here would take the fun out of the game. Games provide a very different service than other AI products. Therefore, more work is needed to understand design guidelines here.
    
%    \item Theme 3: Improving games with the guidelines.
    
%        - Games that explore NN as teammate interaction can benefit from these guidelines. Providing feedback or references to their actions in related to how it affects the AI and its future decisions would be an interesting dynamic to explore. Players would know when the NN should do something and when the human should do something.
        
%        - Being explicit regarding the NN can lead to new interactions. 
        
%    \item Theme 4: Designers and developers interested in NNs can use our framework as a starting point.
    
 %       - Applying our interaction framework allowed us to analyze the gameplay experience as a dialog between the player and the NN. We believe that our framework can be a useful starting point for understanding how \glspl{ann} can affect the gameplay experience and potentially lead to new design opportunities.
        
%        -Showcase gaps from our analysis and examples of how designers and developers can use this for future work.
        
%    \item Theme 5: We are still early in development. There are gaps to fill.
    
%        - Represent the NN and its internal processes in games categorized as NN as competitor or designer may present new interaction opportunities for game designers to consider.
        
%        By looking through games, the current ai guidelines are incomplete to address the missing areas. 
        

%\end{enumerate}

==> prev_submission/archieved_docs/mathiashold.tex <==
\subsection{Why Neural Networks in Games?}

As outlined in section \ref{sec:nn_in_creative_domains}, DNNs can learn any function needed and work well for solving problems in higher dimensions. They can be utilized in countless different ways, and, if done correctly, can reach interesting, creative, solutions.

Interestingly, a large set of recent breakthroughs in the field of AI is by simply taking existing techniques for NNs and combine this in a novel manner or on a new dataset. \todo{Eg. gans, vae, deep fakes, alpha-go}

While the NNs are extremely flexible and work well in higher dimensions compared to many other AI algorithms, they also have several weaknesses. First and foremost, they are data intensive. In order to prevent overfitting to specific circumstances, and instead learn general features, a large, clean, dataset is a necessity. Often, these are hard to obtain, but can for instance be done by collecting player data from many users.

Another symptom of this need for large quantities of data is \emph{user fatique}, which often arise when utilizing HCI and NNs together. As the NN needs many iterations and large quantities of feedback from the user before having reached a well performing solution, the user is at risk of losing interest.

Further, they have a general lack of transparency and predictability. One cannot guarantee the behavior of a NN in the same way one can with a simpler model, e.g. linear regression. Nor can one easily account for the reasoning behind a NNs decision. This lack of \emph{reliability} is part of the reason for the `gap' between the game industry and the AI research community \cite{yannakakis2018artificial}.

Developing NNs require large investments in time and resources. As each developed game is novel in itself, there are also no existing off-the-shelf NN solutions directly applicable to this novel game. This is generally known as the \emph{no free lunch} theorem --- every adoption of a NN in a game will \todo{Seb: I don't think I would classify this as no free lunch} have to be customized to the problem at hand. In addition, there are no prior guarantees for the performance of the developed model. It is for reasons like these the use of NNs in games is yet relatively modest considering the advancements in the field.

Given all of those shortcomings, we did identify categorizations that fit will within certain design spaces. For example, \textit{Online Reward} networks worked very well in pet simulators and for replacing older-styled decision trees in zero-sum competitions. \textit{Offline Content} networks are ubiquitous in PCG endeavours, as they can save developers massive amounts of asset-creation. Lastly, for designers looking to 'wow' players with the most powerful neural networks, an approach like \textit{Semantris} and \textit{Quick, Draw!} is definitely a path forward.

%----------- related work content

%{\color{red}In this section, we % provide an overview of the literature on \gls{ai} in games\todo{now moved to intro}, with a particular focus on NNs. Then, we
%discuss existing work in human-\gls{ai} interaction, including literature on the different ways humans and \gls{ai} interact.[Is this still true?]}

%\subsection{\gls{ai} in Games}

%\todo[inline]{Mathias}
%{\color{red} [An high-level overview of the use of \gls{ai}, especially NN, in computer games.  Budget: 0.5 column.]} 
%\gls{ai} and games have co-evolved ever since the invention of the modern computer \cite{yannakakis2018artificial}. The first applications of \gls{ai} in games focused on search algorithms for creating \gls{ai} agents with the goal of beating a human player \cite{schaeffer1996chinook, turing2009computing}. The games for which the \gls{ai} was created were typically highly restricted, fully observable, turn-based, games like Chess, Backgammon, and Checkers. 

%Recent breakthroughs in the field of Deep Learning, as well as hardware, has allowed the application of \glspl{dnn} for solving increasingly complex tasks. An example of these advancements is \citeauthor{mnih2013playing}'s use of \glspl{dnn} for learning to play several Atari 2600 games, achieving superhuman performance based on raw pixel input \cite{mnih2013playing}.

%Recently, there has been a shift of focus in the application of \gls{ai} in games \cite{yannakakis2018artificial}. The trend is moving away from purely focusing on solving a game with an \gls{ai}-controlled agent, and instead, focus on the use of \gls{ai} to improve if not drive the quality of the player's gameplay experience \cite{riedl2013ai}. 

%This approach refers to using the \gls{ai} for tasks like \gls{pcg}, user preference adaption, and exploration. These applications all include the need for creativity to some extent. While search optimization is an easy task for computers, creativity is far more difficult as it is nearly impossible to quantify in general terms. Nonetheless, a well-defined measure of creativity is needed to avoid a purely exhaustive search, which is computationally infeasible in all interesting domains.  

%Games are particularly well suited for applying \gls{ai} with the aim of generating creativity, as games contain a vast facet of dimensions enabling creativity like sound, multi-agent interaction, visual art, and emotions.



%The first role is \gls{ai} as Actor (for the player), in which the Game \gls{ai} system mediates between the player and the game to create a compelling real time experience. The most common manifestation of \gls{ai} under this paradigm is controlling or managing bots and non-player characters.
%\gls{ai} served the role of an artificial human opponent or playmate, enabling play without requiring other people or filling roles humans would be loathe to fill in a game.
%Game \gls{ai}, the intelligence built into games places a greater emphasis on creating engaging and entertaining experiences for users,
%Most similar to our framework, however we unpack the relationship between the player and \gls{ai} approach, specifically neural networks, to detail the different interactions that occur in these games so designers can better... ?.

%The second role is \gls{ai} as Designer (for the designer), in which the \gls{ai} mediates between a game designer and a single player-game system. Under this paradigm, \gls{ai} systems might procedurally generate game content or adapt the game to particular players to scale the game development process. 
% game designers are responsible for building and defining a game, analyzing how players interact with the game, and iteratively refining a game to achieve a design vision. This refers toG ame adap- tation taken combines content generation and player modeling to enable \gls{ai} designers to tailor games to individual players,

%Finally, \gls{ai} as Producer, in which the \gls{ai} mediates between game producers and a number of systems of players, designers, and games. 
%producers concern them- selves with the entire set of games and game content being made by a company, along with related aspects of managing
%player communities. \gls{ai} Producers mandate a shift from single player experiences within a closed game to long-term player experiences within an open game, understanding a player across multiple games in an ecosystem, and understanding how multiple players interact as an in-game and out-of-game com- munity.
%\gls{ai} Producers also leverage a broader sense of context for enhancing game experiences including the community of players and the real-world context of their activities. \gls{ai} for game production puts a premium on broadening the scope of Game \gls{ai} to better integrate the increasingly pervasive nature of games into how games entertain and engage users.



% \subsection{Neural Networks in Creative Domains}
% \label{sec:nn_in_creative_domains}
% \todo[inline]{Mathias}
% {\color{cyan}{[JZ: Need discussion]}}
% Having a set of domains (games) allowing for creativity to emerge, does not necessarily mean it will. Humans have an intrinsic drive for curiosity and creativity. Neural networks on the other hand, do not. They are created for the sole purpose of minimizing a predefined loss function. However, creativity by definition cannot be predefined. Although neural networks can learn \emph{any} function, theoretically, it does not mean it will do so in practise.

% Hence, we have games which allow for creative behavior, and an algorithm (neural networks) that theoretically can learn anything, the remaining question is how to push for creativity and thus novelty?

% A popular approach is to \todo{add sources} use \gls{hci} (see sec. \ref{seq:human_ai_interaction}) combined with \emph{neuroevolution} for making the \gls{ai} generate solution candidates. The user then selects the most prominent, hence creative, solutions. This interaction can be both directly and indirectly encoded in the domain at hand. This dismisses the need for having to quantify creativity by letting the user decide. 

% It is possible to generate creative artifacts by using only neural networks without the use of human interaction. This is typically done by setting constraints for the generated artifacts, and training the neural network on a dataset of valid solutions. An example of such a constraint is that a generated map should be playable. This requirement, in turn, can be validated using another \gls{ai} agent. XX \todo{source} used the A* algorithm for checking this requirement in Super Mario Bros maps generated by a neural network.

% Eventhough such artifacts are created without any direct user involvement, ultimately, users are the consumers of creativity. The creative artifacts are generated for the user to appreciate. Whether the artifact being a weapon, map, sound, or emotion created by a Neural Network. Therefore, it is also only the user who can evaluate its quality. Consequently, generating creativity without human feedback is unattainable.

%\subsection{How Neural Networks Are Used in Games}
%Before investigating how humans interact with \glspl{ann} and its implications for the player experience\todo{rephrase}, we provide a brief example of how \glspl{ann} can be used in games from a technical point of view. First, to understand how the algorithms work, it is important to have a basic understanding of how \glspl{ann} works in general.

%\glspl{ann} are computational graphs whose structure is inspired by neuroscience and the neural structures found in the brain of animals \cite{hassoun1995fundamentals}. There are a vast variety of different ANNs,  with different structure, training procedure, and application. What they all have in common though, is that they are a mapping $X \rightarrow Y$. This mapping is realized by the computational graph which constitutes a function, $f$. The objective is to find $\widehat f$ which is the desired ground true \emph{target} function. $\widehat f$ is unknown, and $f$ with always be an approximation of it \cite{George1976}. An example of a simple ANN setup is X being a set of images, and Y being a set of labels. Each image is given a label. The objective is to find $\widehat f$, which is the correct mapping from image to label.

%How one finds $\widehat f$ is an ongoing challenge.
%$f$ consists of a set of parameters ($\theta$), in most cases, these are referred to as weights and biases. 
%Some algorithms work with a \emph{fixed} structure for $f$, and simply optimize $\theta$ such that $f(X) \approx \widehat f$. Other algorithms like \emph{neuroevolution} approximate $\widehat f$ through a concurrent search over the structure of $f$ and $\theta$, yielding a set of NNs.



==> prev_submission/archieved_docs/previous_drafts.tex <==



%An effective interaction has been described as one where the AI is understandable and ensures the user is in control of the system \cite{norman1994might}. It is widely accepted that understanding these interactions is crucial step in helping humans overcome any ambiguity \cite{dey2002distributed,amershi2019guidelines} and use AI to its full potential. Additional work has also gone into increasing transparency of the AI to foster more interaction \cite{herlocker2004evaluating,rader2018explanations}.

The ways in which humans interact with AI has been an active topic in HCI research \cite{clarke1993co,desmarais1993advice}. There is certainly no shortage of literature on how to design effective human-AI interaction \cite{amershi2019guidelines}. This body of work emphasizes guidelines to develop interactions that are understandable and enable humans to instruct and lead the system \cite{norman1994might,amershi2019guidelines}. Yet, as AI rapidly advances and its application becomes more common, this in turn, frames more opportunities to explore the relationships that materialize through the user's experience. In other words, literature emphasizes best practices, but more work is needed to understand the dynamics of these interactions from a user's perspective. 

Our emphasis in this paper is to explore the relationships that occur between humans and AI, specifically in games that use neural networks. Therefore, for this section, our focus is to detail existing work regarding how human-AI interact in collaborative settings as these interactions may more appropriately apply to game settings. We then pay particular attention to literature regarding how AI interacts with humans in the domain of games. 

%Specifically, as more dynamic human-AI interactions emerge, understanding the relationships that materialize through the user's experience is crucial to developing future meaningful interactions. As a result, not only must designers consider the usability of the system and how to make interaction understandable, but also the relationships that materialize through the user's experience.
%e to and is integrated into more technologies, the more opportunities emerge to analyze possibilities of dynamic human-AI interactions.  as is applied to different technologies, the less we know how these interactions more it frame new opportunities to apply these approaches to technology,
%and interaction design rapidly advance  how humans interact change how humans interact with AI, the more possibilities of dynamic human-AI interactions emerge.  

%Existing work has addressed different relationships by offering interaction metaphors to describe how humans and AI interact in a creative environment \cite{lubart2005can}. Work has also described and observed social dynamics from human-human interaction be applied to human-computer interaction, such as computers as teammates \cite{nass1996can}, collaborators \cite{wilson2018collaborative,lubart2005can}, and coaches \cite{desmarais1993advice,lubart2005can}.
%By using these metaphors, designers are able to understand the role of the computer to potentially foster these human relationships during the users experience with the computer. 

%there is a need to further understand how humans and AI interact outside of a tool setting. Further, using interaction metaphors to redefine and advance our understanding of the relationships that occur between humans and AI. Therefore, for this section, our focus is to detail existing work on interaction metaphors for human and AI relations, with a particular focus on how AI interacts with humans in the domain of games. 


%Work in HCI, correctly so, prioritizes the human and the feeling of being in control. However, most of this work focuses on how to enable humans to instruct or lead the system \cite{norman1994might,amershi2019guidelines}. As more opportunities to interact collaboratively with AI emerge, there is a need to further understand how humans and AI interact outside of a tool setting \todo{need reference}\cite{}. 
%Existing research has observed social dynamics from human-human interaction be applied to human-computer interaction. They have described this interaction this using a variety of interaction metaphors, such as computers as teammates \cite{nass1996can}, collaborators \cite{wilson2018collaborative,lubart2005can}, and coaches \cite{desmarais1993advice,lubart2005can}. By using these metaphors, designers are able to understand the role of the computer to potentially foster these human relationships during the users experience with the computer. 
%Most relevant to this paper, we highlight work that discusses how human-AI interact in these dynamic settings as they may more appropriately apply to game settings.
%These sources usually investigate the ways humans interact and respond to AI in a variety of settings such as a teammate, collaborator, and coach.

In the research area of Creative Support tools, growing efforts have looked into {\em creativity support tools} from an HCI point of view. Lubart \cite{lubart2005can} proposed four interaction metaphors of how computers can be partners in the creative process --- computer as nanny (managing and support), pen-pal (supporting communications between collaborating individuals), coach (using creativity enhancement techniques), or colleague (human-computer cooperation during idea production). Among them, colleague is the most ambiguous and requires synergistic hybrid human–computer systems \cite{lubart2005can}. These interaction metaphors advance the design space by providing designers and researchers a perspective on how computers can support or contribute to human's creative work.


\textcolor{blue}{unsure if this work is relevant}
Other work has also explored how humans and AI can work together as collages in the workplace. Wilson et al. \cite{wilson2018collaborative} propose an interaction cycle between humans and AI to detail the possibilities of human-AI collaboration to improve work performance. Through the lens of \textit{humans assisting machines} and \textit{machines assisting humans}, Wilson et al., describe different examples to help business leaders understand both human and AI's complementary strengths and identify collaborative opportunities. They describe that humans help train and explain tasks to computers and, in turn, computers can amplify creativity and assist in decision-making processes by providing the right information at the right time-- such as helping humans spark ideas or thoughts that they may not have considered initially. 

Research has also investigated how human-human interactions can also be applied to human-computer interactions \cite{nass1996can,desmarais1993advice}. For example, Nass et al. \cite{nass1996can} determined that humans will readily form a typical human relationship, such as forming team relationship, with computers. They conducted an experiment to investigate how humans perceive computers as teammates by manipulating the computer's identity and interdependency to create a team affiliation with the computer. The results indicated that convincing humans that they are a part of a team with a computer is surprisingly easy and that the user's perception of the interaction is what is important to facilitate teamwork. The data also shows that the effects of being in a team with a computer are the same as the effects of being in a team with another human. Their data concluded that humans in the interdependence conditions perceived the computer to be more similar to themselves, saw themselves as more cooperative, and were more open to influence from the computer \cite{nass1996can}. 

It is clear that humans and AI can interact in dynamic ways that are outside the typical tool setting \cite{nass1996can,desmarais1993advice,wilson2018collaborative}. Further describing these interactions can lead to new design considerations that can emulate existing human-human interactions \cite{lubart2005can}. Therefore, in our work, we aim to ...

\subsubsection{Human and AI Interaction in Games} 
The application of AI in games has recently shifted from solving and playing games to developing, if not entirely, producing the player's experience \cite{riedl2013ai}. As games have become increasingly more persistent, game AI plays a significant role in extending playability \cite{} and delivering enjoyable experiences to the player \cite{riedl2013ai}.

Game AI has extended the playability of a game through procedural content generation (PCG), which generates content for the player. AI has also been used to create engaging interactions with players by playing the roles of agents or NPC characters and mediating the entire experience through drama managers. As a result, AIs new involvement in the production of player experiences has created new ways for humans and AI to interact. 

Existing work has developed interaction metaphors to further detail the role AI plays in the game development process. Riedl et al. \cite{riedl2013ai} group game AI into three roles that AI take on in the creation and delivery of gameplay experiences. Each role individually targets: players, designers, and producers, which aim to define how AI assist these human stakeholders. The three roles are as follows: AI as an Actor, describes how AI mediates between the player and the game itself.  This refers to how AI serves as a playmate to the player, creating engaging experiences by controlling or managing bots and non-player characters. AI as a Designer, describes how AI mediates between a game designer and the game system. This refers to how the designer combines content generation and player modeling to enable the AI to tailor games to individual players. Lastly, AI as a Producer, describes how AI mediates between producers and many systems of designers, users, and games. In their metaphor, producers concern them- selves with the managing entire set of games and game content made by a company, along with related aspects of managing players. This refers to how AI can assist in understand a player across multiple games and how multiple players interact as in-game and out-of-game community \cite{riedl2013ai}.

Riedl et al. \cite{riedl2013ai} metaphors provide a high-level understanding of the different roles AI take on to assist a variety of different stakeholders in game production. This work is the most closely related to this paper's contribution. However, what sets our work apart, is that we emphasize and unpack the relationship between the player and the AI. Our goal is to classify the existing design space of how AI, specifically neural networks, can be used as game mechanics in terms of its relationship to the player.


%%------- NN specific old text 6-3-2020
%the creature represents the neural network on the surface and does not reference the network's presence or its capabilities in the UI. 
%To contrast, other games highlight the existence of the NN in the core gameplay UI. Two games,\textit{How to train Your Snake} \cite{snake} and \textit{Idle Machine Learning Game} \cite{idle} were categorized as NN-Specific and directly referred to the network in the core gameplay UI. These games also made the network's capabilities and modes of interaction available through the surface interface.
%Therefore, players potentially were more aware of the neural network and what it is capable of accomplishing.  

%For example, \textit{How to Train your Snake} \cite{snake} is a web-based incremental game based on the game Snake, where a line (or snake) maneuvers a limited space to gather food. The snake continuously grows in length while its tail becomes a primary obstacle to avoid. In this version, the player is given four different snakes that represent four different neural networks.  The objective for each snake is to survive by eating the food and not running into themselves. The player's primary goal is to steer the NN by purchasing various upgrades and observe the consequence when prioritizing different neural network parameters. 

%\textit{How to Train your Snake} \cite{snake}  was  categorized as NN-Specific because the core gameplay UI explicitly refers to the neural network and represents the system's capabilities through various upgrade mechanics that include technical terminology. Further, by making these capabilities available to the player, the gameplay consists of exploring the NN parameters and the different ways to steer the behavior of the surface snakes. These capabilities are directly reflected in the game's UI.

%Teammate
%Of these five games, four were categorized as NN-Specific and directly referred to the network in the core gameplay UI. These games made the network's presence explicit through the UI, which further highlights its role as a teammate during gameplay since both player and NN are needed to progress in the game.

%In another example, the player collaborates with a neural network by helping it train for fights against other AI agents. \textit{Machine Learning Arena} is a single-player fighting game where the player performs fighting actions for the NN agent to copy and learn to use during boxing matches against other AI-agents. The player's objective is to work with the NN to train it to learn how to punch and dodge incoming attacks. When done training, the NN fights other AI agents on its own while the player observes. This interaction is collaborative because the player needs the network to compete in the match, and the network can only be successful with the player's training. 

%The distinction in this example, compared to\textit{Evolution}, is the UI further describes the progress of the NN in terms of coping and learning through displayed stats and UI meters. The combination of a copy and reward meter indicates that the agent is learning from the player's actions and visualizes the impact of the actions performed.

%---------- Nn-limited old text 6-3-2020


%Further, \textit{Creatures} \cite{grand1997creatures} is also categorized as NN-Limited as they did not refer to the NN in the core gameplay UI. However, they use technical terminology in the tutorial and menus, which refer to the evolution and generations of the creatures, therefore indicating the existence of the NN.

%----
%competitor 
%In contrast, only one game provided limited UI references to the neural network in the menu, but did not address the network in the core gameplay loop.

%-----
%designer
%To contrast, two games \textit{AI Dungeon} \cite{aidungeon} and \textit{Darwin's Avatar} \cite{lessin2015darwin}, games were categorized as NN-Limited, as they did not refer to the neural network in the core gameplay UI, but did indicate the existence of the NN through tutorials \cite{aidungeon} or through game menus \cite{lessin2015darwin}. For example,  \textit{Darwin's Avatar}, is a multiplayer racing game where players learn to move and race various creatures with arbitrary keyboard controls, whose controls are designed by a neural network. Each creature's morphology, consists of various limbs and muscles, and is evolved together with a neural network. The players must learn how to control the creature's movement while racing against other players. Players can also race against the neural network that was used to train the creature; however, this is not the main interaction of the game. As a result, the neural network further develops new combinations for players to learn, keeping the experience new for each time the player races. 
%\textcolor{red}{Need to check this paragraph with Sebastian.}

%------- NN-Agnostic old text 6-3-2020
%apprentice
%Two games, \textit{Black & White} \cite{wexler2002artificial} and \textit{Hey Robot} \cite{hey}, were categorized as NN-Agnostic and did not refer to the neural network in any of the UI. As a result, the neural network is often represented as a character or object within the game.  For example, \textit{Black & White} is a single-player computer game where the player plays as a god who rules over several islands populated by villagers. The goal of the game is to gain control over all the islands and defeat Nemesis, another god who wants to take over the world. The player interacts with these villagers through an on-screen hand, which can be used to cast miracles and perform other actions. The player is assisted by an avatar creature, which is a neural network. The creature helps carry out the player's instructions and whose behavior changes based on how the player treats the creature. Teaching the creature is performed by a pet or slap game mechanic to instruct what and when the creature should eat and how to attack or impress enemy villages. 

%The UI in \textit{Black & White} \cite{wexler2002artificial} does not make the NN known to the player, as the creature stands in place of the NN. Therefore, the player may not be aware of the system's capabilities or how their actions influence the output of the NN. This interaction differs from \textit{Creatures} \cite{grand1997creatures} as the player may be more aware that the system is learning through the terminology used in the game's UI. Thus, potentially making players more mindful or selective of their actions as they impact the direction of the output. 

%------------
%competitor 
%Games in this category give the neural network a better approximation of the player's strategy, leading to a more robust and challenging gameplay experience.  In light of creating a more human-like opponent, three of the four games were categorized as NN-Agnostic and did not reference the neural network in the UI. As a result, the NN is represented as an enemy unit \cite{rabin2015game} or challenger, such as the drivers in the \textit{Forza series} \cite{takahashi_2018} and \textit{MotoGP19} \cite{moto}.

%----
%Designer
%\textit{Petalz} \cite{risi2015petalz} does not reference the existence of the network in the game UI and was categorized as NN-Agnostic. As a result, players may or may not be aware of the network or how their selections of flowers may impact future generations of during gameplay. Further, two other games, \textit{Audio in Space} and \textit{GAR}, were also categorized as NN-Agnostic. 
%These games did not indicate the richness of the underlying system through its UI; therefore, players may not be aware of how their actions impact the decisions or content of the network's output.





%Section 4 6-3-2020
%------------------------------------------------

%\subsection{Apprentice}
%Players selectively breed Norns with desired characteristics and, in turn, teach each Norn the desired behavior by positive (petting), negative (striking) reinforcement and text input. 
%When a new creature hatches, players must reteach the creature and figure out, from past experiences with prior generations, what combination of actions and traits will keep them alive the longest. 
%The life cycle of each Norn encourages an explorative gameplay cycle of trial and error through what combination of gameplay actions and creature traits is best to keep them alive the longest. Additionally, the NN is purely lead by the direction of the player and has no explicit game play goal that is shared with the player. It simply follows the lead of the player. 


%\textit{Hey Robot}, another \textit{apprentice} example with a different structure, is a word association game in which players attempt to get Amazon's Alexa to utter a specific word. In this case, the player must weigh different verbal inputs to get the desired word or output needed from the device.


%the modes of interaction made available through their surfaces encourage a process of play. 
%However, this game did not reference the neural network in their UI. As a result, the complexity of the underlying system is hidden and players may not be aware how the system is using the players input and what the possible   represent their internal system 
%is accomplished by creating a simulated world, processes for behavior in and of the world, and characters and objects that populate the world. , the surface of a work of digital media is not transparent—it does not allow for direct observation of the data and process elements created. 

%Of the 6 games in this category, four games made the player aware of the neural network during gameplay. Add more... 
%\textcolor{blue}{I feel like this is important, but I'm not sure this is adding anything to results.}
%This awareness can further orient the player's gameplay and actions toward understanding the capabilities of the system.
%Computer as an \textit{apprentice} refers to the neural networks that take on a subordinate or impressionable role during gameplay that players actively lead to a desired output. Players interact with these networks by instructing and molding the network through direct interaction, such as telling the neural network what is good or bad behavior, or indirectly, when the neural network observes the player's gameplay to shape its output.

%Of the 16 games, six games fell into this category: \textit{Black & White},\textit{Creatures}, \textit{Hey Robot}, \textit{How to Train your Snake},\textit{Idle Machine Learning Game}, and \textit{Semantris}. In the majority of these instances, the neural network is not aware of the game's objective, but rather the player is trying to lead the neural network to produce a specific output. Only two games, \textit{Hey Robot} and \textit{Semantris} indicate that they are using a neural network and made this known to the player during gameplay. 


%\subsubsection{Neural Network as a Competitor}
%%    \item \textit{Competitor}: Neural networks as a competitor occur when the neural networks take on the role of a challenger during gameplay. This interaction emphasizes the player's role as a rival of the neural network whose strategy is observed in order for the neural networks to adapt it's output. Neural networks interact with the players through observing player actions and, in turn, adjusting to accommodate the player's input or strategy to ensure a competitive gameplay experience.

%Neural networks as a \textit{competitor} occur when the player and the neural networks take on the role of rivals during gameplay. This interaction emphasizes the player's gameplay whose strategy and actions are observed in order for the neural networks to adapt it's output to counter the player. Neural networks interact with the players by adjusting its output to accommodate the player's input to ensure a competitive gameplay experience. 

%Of the 20 games, four games were categorized as a competitor. These games implement this interaction by providing the player with a more human-like opponent, which adapts or counters the player's actions as a human opponent would in real-life. As a result, this creates a more realistic challenge that evolves with the player throughout the experience. For example, \textit{Supreme Commander 2} \cite{rabin2015game}  is a single-player real-time strategy game where players customize and command an army platoons in battle against the AI, which is a neural network. The goal is to kill a specific unit in each army to win the battle. As the player customizes their army, the neural network weighs the player's unit composition against its own and makes tactical battle decisions, such as how its army will respond, which enemy to target first, or when to retreat. As a result, the NN produces a gameplay experience more similar to playing against a human opponent, where an opponent would also make similar decisions and respond accordingly.  A key distinction in this category is that the players counter the player's actions. It uses these actions to defeat or contrast the player in some way as to provide a challenge.

%While the network does not "learn" from the player, it's decisions are swayed by the player's actions. Therefore, enemy units make better, more self-preserving decisions than previous implementations of the AI. This advanced self-preservation produces a gameplay experience more similar to playing against a human opponent.

%Games in this category give the neural network a better approximation of the player's strategy, leading to a more robust and challenging gameplay experience.  In light of creating a more human-like opponent, three of the four games were categorized as NN-Agnostic and did not reference the neural network in the UI. As a result, the NN is represented as an enemy unit \cite{rabin2015game} or challenger, such as the drivers in the \textit{Forza series} \cite{takahashi_2018} and \textit{MotoGP19} \cite{moto}.
%In contrast, only one game provided limited UI references to the neural network in the menu, but did not address the network in the core gameplay loop.


%For example, \textit{Supreme Commander 2} did not highlight the neural network presence in the UI or use technical terminology. Players' focus, therefore, remains on the game objective, and the UI did not refer to the interaction occurring behind the surface battle. 

%In contrast, only one game provided limited UI references to the neural network in the menu, but did not address the network in the core gameplay loop. The \textit{Forza} game series is a racing simulator in which players can customize and race cars. Players can select vehicles and their drivers and choose between racing other players or drivatars. In this case, the drivatar is a neural network that continues to train via reinforcement learning based on their placement in previous races. That means the NN adapts both to the player and the other "drivatar" controlled racers.
%that observes the player's performance from completed races and attempts to closely match the player's performance to ensure an appropriate challenge. 
%The game's menu explicitly refers to the drivatar as a NN Agent and explains that the player's data is used to train the agent. It also states that the drivatar is trained to compete similarly to the player. However, this is only accessible by the player in the menus and is not present during the race. 

%Providing players with references to the network and its objective can potentially further create a dialog between the player and the neural network. If the game UI makes the system known, the player could potentially adjust or modify their behavior to train the drivatar to behave in a particular way to compete in future races. 


%Of the 16 games, three games fell into this category: \textit{Abbratoir}, \textit{Forza Car Racing}, and \textit{Supreme Commander 2}. In each of these cases, the neural network was not made explicit to the player during gameplay. In fact, neural networks were implemented into each of these games simply to improve upon and replace already-existing competitive AI structures such as decision trees. Despite not being aware of the network, the player does witness the neural networks improvement over time as it retrains with data specific to each player.

%\subsubsection{Neural Network as a Designer}
    
%    \item \textit{Designer}: Neural networks as a designer occur when the neural networks take on the role of a creator or author during gameplay. This interaction emphasizes the player's role as a client who actively interacts with the results of the networks creation. The neural network generates content for the player based on direct player inputs or by indirectly analyzing a player's preferences during gameplay. As a  result, neural networks extend playability of the game by providing content variety that is unique to each player.
    

%Neural networks as a \textit{designer} occur when the neural networks take on the role of a creator, and the player takes on the role of the client during gameplay. This interaction extends the gameplay experience by the neural network generating new or tailored content for the player. As a result, neural networks extend the playability or gameplay experience by continuously generating content for the player. 
%The neural network generates content for the player based on direct player inputs or by indirectly analyzing a player's preferences during gameplay. 

%Of the 20 games, five games were categorized as a designer. These games implemented this interaction by providing the player with a varied experience which is influenced by the players gameplay actions. A key distinction for this category, is that the goal of the NN is to extend the game with new or tailored content to provide the player with fresh experiences. 


%For example,  \textit{Petalz} \cite{risi2015petalz}, is a social media game where players arrange and nurture a balcony of flowers. Players can plant, water, and breed new flowers and sell them on a marketplace. If the player chooses, they can also help their friend's flowers by watering their garden. A neural network generates each flower (shape and color) based on the player's selection of flowers to breed or cross-pollinate. The underlying neural networks mutate and crossover each flower generation, allowing each player to customize their flowers to their liking. As a result, the NN extends playability by providing flowers that match the preferences of the player.
%these actions implicitly reinforces the neural network on the player's preferences and, thus, dictates what flowers the network produces. Therefore, it extends and customizes the flowers for each player. 

%\textit{Petalz} \cite{risi2015petalz} does not reference the existence of the network in the game UI and was categorized as NN-Agnostic. As a result, players may or may not be aware of the network or how their selections of flowers may impact future generations of during gameplay. Further, two other games, \textit{Audio in Space} and \textit{GAR}, were also categorized as NN-Agnostic. 
%These games did not indicate the richness of the underlying system through its UI; therefore, players may not be aware of how their actions impact the decisions or content of the network's output.

%To contrast, two games \textit{AI Dungeon} \cite{aidungeon} and \textit{Darwin's Avatar} \cite{lessin2015darwin}, games were categorized as NN-Limited, as they did not refer to the neural network in the core gameplay UI, but did indicate the existence of the NN through tutorials \cite{aidungeon} or through game menus \cite{lessin2015darwin}. For example,  \textit{Darwin's Avatar}, is a multiplayer racing game where players learn to move and race various creatures with arbitrary keyboard controls, whose controls are designed by a neural network. Each creature's morphology, consists of various limbs and muscles, and is evolved together with a neural network. The players must learn how to control the creature's movement while racing against other players. Players can also race against the neural network that was used to train the creature; however, this is not the main interaction of the game. As a result, the neural network further develops new combinations for players to learn, keeping the experience new for each time the player races. 
%\textcolor{red}{Need to check this paragraph with Sebastian.}




%For example,  \textit{Darwin's Avatar}, is a multiplayer racing game where players learn to move various creatures to the finish line or until a time limit is reached. 
%are presented with creatures whose morphology, consisting of various limbs and muscles, evolve together to learn how to move by together with a neural network.  
%Using arbitrary controls on a keyboard, players are tasked with moving and racing the creatures morphology against another player by taking control of one of the evolved creatures.
%Players can also race against the neural network that was used to train the creature.







%Of the 16 games, three games fell into this category: \textit{AI Dungeon}, \textit{Darwin's Avatar}, \textit{GAR}, and \textit{Petalz}. In these games, the network's priority is to create an interactive and varied experience procedurally. Only one game, \textit{AI Dungeon}, made the network explicit to the player; for the most part, the "magic" of the network was part of the player experience, and thus was hidden from the player.



%\subsubsection{Neural Network as a Teammate}

%    \item \textit{Teammate}: Neural networks as a teammate occur when the neural networks take on the role of a colleague during gameplay. This interaction emphasizes the player's role as an ally or collaborator who works with the neural network toward a shared goal. In this case, the player still takes the lead by directing what the neural network interacts with; however, in this case, the neural network offers up skills that are needed to advance in the game.  As a result, both player and neural networks are necessary to be successful in the game and work together to achieve the objective.

%Neural networks as a \textit{teammate} occur when the neural networks take on the role of a colleague during gameplay.  This interaction emphasizes the player's role as an ally or collaborator who works with the neural network toward a shared goal. In this case, the player still takes the lead by directing what the neural network interacts with; however, in this case, the neural network offers up skills or mechanics that are needed to advance in the game.  

%Of the 20 games, five games were categorized as a teammate. These games implemented this interaction by providing the player with an objective that they can not successful without collaborating with the neural network. For example, \textit{Evolution} \cite{evolution}, is a single-player simulation game where players build a stick-figure-like creature, through placing bones,  muscles, and joints. Once assembled, the player can submit the creation to the neural network and observe their creature evolve. The NN performs tasks, such as which combination of the creature's morphology leads to running, jumping, and climbing.  From there, the player can stop the simulation and further improve on its design. This interaction creates a collaborative cycle between the player and the neural network through the building and training of a creature to perform various tasks.  A key distinction for this category, is that both the player and the NN share a gameplay goal and both are needed to be successful. 


%Of these five games, four were categorized as NN-Specific and directly referred to the network in the core gameplay UI. These games made the network's presence explicit through the UI, which further highlights its role as a teammate during gameplay since both player and NN are needed to progress in the game.

%In another example, the player collaborates with a neural network by helping it train for fights against other AI agents. \textit{Machine Learning Arena} is a single-player fighting game where the player performs fighting actions for the NN agent to copy and learn to use during boxing matches against other AI-agents. The player's objective is to work with the NN to train it to learn how to punch and dodge incoming attacks. When done training, the NN fights other AI agents on its own while the player observes. This interaction is collaborative because the player needs the network to compete in the match, and the network can only be successful with the player's training. 


%The distinction in this example, compared to\textit{ Evolution}, is the UI further describes the progress of the NN in terms of coping and learning through displayed stats and UI meters. The combination of a copy and reward meter indicates that the agent is learning from the player's actions and visualizes the impact of the actions performed.


















%Section 3 6-3-2020
%--------------------------------------
%Based on our two research questions, they coded the collected data on the following questions: 1) What role does the NN play in the overall game system? 2) What kind of neural network does the game use? 3) How does the player interact with the neural network? 4) Does the neural network evolve during the game? 5) How, if at all, does the game reference the neural network in the game UI? Each question was recorded and shared with the group. The two researchers independently coded  classifications and shared their findings with the group for further discussion. 

%Step 2: As a group, the same researchers from step one, discussed each other's preliminary classifications and revised them after exchanging feedback. Upon agreement of the classifications, both researchers classified five games independently and then presented their results to the group. If a disagreement emerged regarding a game's classification, the game would be reanalyzed by both researchers and then resolved through discussion. Once the classifications were clear, the rest of the games were coded separately. 

%\subsection{Analytical Framework}
%\todo{Seb: Are there others surveys that use similar types?} 
%Two classifications were derived from this analysis: (1) how does the player interact with the neural network, and (2) how does the neural network interact with the player. For the first classification, we address this through four interactions metaphors: computer as an \textit{apprentice}, \textit{competitor}, \textit{designer}, and \textit{teammate}. We define each of these elements below to detail the player-NN relationship during gameplay. (1) what are the playey NN interactions used in these games, (2) how are NN used to support player experience in these days

%\begin{enumerate}
%    \item \textit{Apprentice}: Neural networks as an apprentice occur when the neural networks take on the role of a learner or pupil during gameplay. This interaction emphasizes the player's role as a mentor who actively leads and instructs the neural network to a desired goal. In this case, the neural network is directed toward an unknown player-developed goal where the neural network is guided over time through the player's gameplay. This can occur through direct interaction, such as telling the neural network what is good or bad behavior, or indirectly, when the neural network observes the player's gameplay to shape its output.

%    \item \textit{Competitor}: Neural networks as a competitor occur when the neural networks take on the role of a challenger during gameplay. This interaction emphasizes the player's role as a rival of the neural network whose strategy is observed in order for the neural networks to adapt it's output. Neural networks interact with the players through observing player actions and, in turn, adjusting to accommodate the player's input or strategy to ensure a competitive gameplay experience.
    
%   \item \textit{Designer}: Neural networks as a designer occur when the neural networks take on the role of a creator or author during gameplay. This interaction emphasizes the player's role as a client who actively interacts with the results of the networks creation. The neural network generates content for the player based on direct player inputs or by indirectly analyzing a player's preferences during gameplay. As a  result, neural networks extend playability of the game by providing content variety that is unique to each player.
    
%    \item \textit{Teammate}: Neural networks as a teammate occur when the neural networks take on the role of a colleague during gameplay. This interaction emphasizes the player's role as an ally or collaborator who works with the neural network toward a shared goal. In this case, the player still takes the lead by directing what the neural network interacts with; however, in this case, the neural network offers up skills that are needed to advance in the game.  As a result, both player and neural networks are necessary to be successful in the game and work together to achieve the objective.

%\end{enumerate}

%Additionally, we further subdivide this categorization based on how these games, if at all, highlight the neural network's existence through the user interface (UI). We use this distinction to showcase which games made the network known to the player, as this can indicate potentially different player-NN interactions and new areas for design work. In an effort to display this distinction, we create a 3 level scale which includes: \textit{NN-Specific UI}, \textit{NN-Limited UI}, and \textit{NN-Agnostic UI}. The definitions of this scale is as follows:

% \subsection{Classifications}

% Two classifications were derived from our observations that aim to address two research questions: 1) What are the player NN interactions used in these games? and 2) How is the NN used to support the player experience? As a result, two tables were created to categorize 20 games into the following framework. 

% We address the player-NN interactions with four interaction metaphors: computer as an \textit{apprentice}, \textit{competitor}, \textit{designer}, and \textit{teammate}. We define each of these interactions in section \ref{results} and detail how these interactions occur during gameplay. 

% Additionally, we further subdivided these interactions based on how these games, if at all, highlight the neural network's existence through the user interface (UI). We use this distinction to showcase which games made the neural network known to the player through the UI, as this can indicate different interactions and new areas for design work. 

% As a result, we created a three-level scale to describe where the neural network was made known in the game's UI. We consider games that use the term "neural network" or "AI" and technical terms, such as "generation," "population", and "evolution" in the game's UI to be a reference to the neural network. Our levels include 1) \textit{NN-Specific UI}, which refers to the games that highlight the NN in core gameplay UI. 2) \textit{NN-Limited UI}, which refers to games that only highlight the NN in non-essential gameplay UI, such as title screens, help menus, etc. 3) \textit{NN-Agnostic UI}, which refers to games that do not reference the NN in the game UI.

%\begin{enumerate}
%   \item \textit{NN-Specific UI}: This refers to the UI that exhibits the highest level of existence of the neural network. We categorize games in this level that explicitly use of the term "neural network" or "AI" in the UI. Or use technical terms during gameplay, such as “generation” "population", "evolution", etc. This level only includes games that highlight the network in core gameplay UI that players must use or interact with to play the game.
    
%    \item \textit{NN-Limited UI}: This refers to the UI that exhibits the lowest level of existence of the neural network. We categorize games in this level that reference the neural network in non-essential gameplay UI, such as title screens, help menus, etc. This level only includes games that do not highlight the neural network in the core gameplay UI. 
    
%    \item \textit{NN-Agnostic UI}: This refers to the UI that exhibits the no level existence of the neural network inside the game. We categorize games in this level that do not reference the neural network during gameplay.
%\end{enumerate}

% We then address how the neural network supports the player experience by detailing three components of the neural network 1) its architecture, 2) how it receives player data, and 3) what the output is in terms of the player experience. First, we examined whether or not the NNs retrain during gameplay or prior to gameplay to indicate how the NN interact with the player's gameplay. We refer to this distinction as \textit{Online} or \textit{Offline} learning. Secondly, we subdivided \textit{Online} and\textit{Offline} learning into two categories, \textit{Behaviors} and \textit{Content}, which refer to the NN's output, as this indicates what the NN provides the player during gameplay. Thirdly, we identified four ways the network receives data from the player, which refers to what player actions the NN observes or collects from the player to dictate how it will respond in the game. We identified these methods as \textit{Rewards, Preferences, Natural Language Processing,} and \textit{Image Analysis}. The definitions are detailed in section \ref{results} and detail how these support different player experiences.

%\begin{enumerate}
%   \item \textit{NN-Specific UI}: This refers to the UI that exhibits the highest level of existence of the neural network. We categorize games in this level that explicitly use of the term "neural network" or "AI" in the UI. Or use technical terms during gameplay, such as “generation” "population", "evolution", etc. This level only includes games that highlight the network in core gameplay UI that players must use or interact with to play the game.
    
%    \item \textit{NN-Limited UI}: This refers to the UI that exhibits the lowest level of existence of the neural network. We categorize games in this level that reference the neural network in non-essential gameplay UI, such as title screens, help menus, etc. This level only includes games that do not highlight the neural network in the core gameplay UI. 
    
%    \item \textit{NN-Agnostic UI}: This refers to the UI that exhibits the no level existence of the neural network inside the game. We categorize games in this level that do not reference the neural network during gameplay.
%\end{enumerate}



%For the second classification, we address three components of the neural network 1) the details about the architecture of the neural network, 2) how the network receives player data, and 3) what the resulting output is for players during gameplay. Regarding the network's architecture, we examined whether or not the networks retrain during gameplay to learn more about individual player behavior. We refer to this distinction as \textit{Online} or \textit{Offline} learning. These definitions are as follows:


%   \begin{enumerate}
%        \item Online: Online neural networks retrain while or immediately after interacting with the player. This retraining is an effort to "learn" something about each individual player, whether that be their preferences, tendencies, and/or strategies. This lends an effect of "evolution" to the NN-controlled agent.
        
    
%        \item Offline: Offline neural networks are defined as trained networks that do not undergo further retraining while or after interacting with individual players. This static behavior means that the network performs identically for all players. These networks are uniquely well-suited for content creation and open-ended inputs in which the player can say or draw anything for the network to examine. 

    
%    \end{enumerate}
    
%Secondly, we further subdivide \textit{Online} and\textit{Offline} learning into two categories, \textit{Behaviors} and \textit{Content}, which refer to the neural network's output. The output, in this case, is how the network responds to player input and provides \textit{Behaviors} or \textit{Content} during gameplay. The definitions are as follows:
%\begin{enumerate}
%    \item Behaviors: Neural networks often output a behavioral decision for the agent they control. That is, the neural network takes player and/or game-world data as an input and then decides on the action that the agent should perform.
    %Seb: Commented this out. Not always finite set 
    %"on a behavior from a finite list of options, based on that input . "
%    These neural networks are often implemented as more advanced "AI" solutions in situations where finite state machines and/or hard-coding every possible scenario was used previously. %This decision can occur every few fractional seconds, like a neural-network controlled agent in a racing game, or based on when the neural network and player directly interact with one another like in real time strategy games. 
    
%    \item Content: Neural networks can also output content for the player. This content might be the focus of the game, like when the player and a neural network collaborate on an objective, or it might be a tertiary gameplay experience like dynamic background music generation. The main distinction is that the network creates content that the player interacts with. This form of neural network output can help procedurally generate highly-tailored content to increase replayability.
%\end{enumerate}

%Lastly, we identified four ways in which the network receives data from the player. This refers to what player actions the network observes and uses to dictate how it will respond in the game. We identified these methods as: \textit{Rewards, Preferences, Natural Language Processing,} and \textit{Image Analysis}. The definitions are as follows:

%\begin{enumerate}
%    \item Rewards: Reward input is the concept of implementing a gamified version of reinforcement learning. This general architecture applies a point value to every action/outcome for a given activity and incentives the neural network to reproduce actions associated with higher point values. The gamification of this concept can allow the player to instruct the network through rewards and punishments as they see fit.
    %, rather than through the traditional implementation of a heuristic. 
    
%    \item Preferences: Preference input is the concept of learning from the player based on their gameplay preferences. These preferences can be actively or passively conveyed to the neural network. In our research, methods based o n interactive evolution are the most common in this category. In terms of design, preference inputs can be utilized in both "AI" advancement for decision making as well as in PCG.%MORE EXPLANATION IF WE WANT This evolution to solve a problem is contingent on a fitness function that calculates the quality of a genome, with higher scores coinciding with a better ability to solve a given problem.
    %Seb: More accurate to say it's interactive evolution. Neat is just one method to evolve neural networks 
    %"NEAT neural network training architecture and its various offshoots "
 %    

    
%    \item Natural Language/Text: Natural Language input is the concept of open-ended text or spoken-language being the player's input to the neural network. All of these games designed their gameplay around an already-existing and very advanced neural network. It's important to note that the main feature is the open-ended nature of the player's input -- that is, they can say or type anything and expect a reasonable response in return. These projects all create the rules and functionality of their game based on the network's capabilities.
    
%     \item Image: Image input is the concept of player's giving an open-ended image to the neural network. Like the \textit{Natural Language} games, this category is also defined by the gameplay being fundamentally designed around accommodating a preexisting and advanced neural network.
% \end{enumerate}


%--------------------------------------







Section 4
%In this case, reinforcement refers to networks that continue to retrain based on new data. For example, in \textit{Black & White} the neural network takes the form of a God. The God learns new activities and mechanics naturally as it explores the island and observes its villages; however, the player can directly impact the model's retraining by giving positive and negative reinforcement after actions via a pet-or-slap mechanic. In another example, \textit{How to Train Your Snake}, the player's interaction with the neural network is obscured by the gameplay, but is no less impactful on the neural network's retraining. \textit{How to Train Your Snake} consists of four separate neural networks training to improve at the classic phone game \textit{Snake}. Players are allowed to modify each network's parameters via various in-game upgrades, thus allowing the models to differentiate themselves over time. For example, the player can double the value of food, thus increasing the positive feedback given when a model's snake reaches the food.

%A Tamagotchi-style game in which the player interacts with virtual pet creatures in an object-filled terrarium. The pets are each controlled by independent AI agents implemented via a neural network inspired by biology. Creatures have drives (hunger, fear, fatigue, etc.) and perception of immediate environment.  They mature over the course of a few hours and eventually die, potentially reproducing in the meantime to create a new generation constructed via genetic algorithm.Player interacts with an NPC creature whose behaviors, perception, and cognition are governed by the NN. Players can provide positive (petting) and negative (striking) reinforcement. NN as co-author of the agent’s personality based on player reinforcement. NN for PCG construction (i.e., believable NPC behavior).

%\subsubsection{Player Input}
%Two games--\textit{Hey Robot and Semantris} were categorized as using offline learning. These neural networks are pretrained and static--meaning no further retraining will occur when interfacing with the player. Rather, verdicts and/or results are rendered from the network solely based on player input. This interaction is both direct, and the player is fully aware it is interacting with a neural network. For example, \textit{Hey Robot} is a card-and-video game in which players are given a keyword on their turn. They then have one attempt to get Amazon's Alexa (or Google's Home) voice assistant to utter the keyword, without uttering the keyword in their prompt. This direct interaction, coupled with the explicit knowledge that the player is interacting with a neural network, makes these games unique.

%Cut This?
%In another example, Black & White, players play as a god and interact with a creature, who carries out the player's instructions and whose behavior changes in reaction to the player's actions. Players indirectly interact with the neural network by their gameplay. 



%\subsubsection{Observational}
%\textit{Supreme Commander 2 and Abbratoir} both utilize dynamic neural networks that retrain by passively observing player data.\todo{Seb: Do you mean supervised learning when you say passively observe the player?} These networks interact with the player by controlling enemy decisions in a more dynamic way than a traditional, static decision tree. This usage of player data means that the interaction between the network and the player is primarily indirect. As an example, \textit{Abbratoir} is an endless tower defense game in which the player is tasked with protecting their land from invading robots. Rather than increasing the difficulty solely through adding more enemy units, \textit{Abbratoir} instead opts to let a dynamic neural network control enemy decisions. This allows for the neural network to pick up and exploit tendencies and tactics the player has become overly reliant on.

%\subsubsection{Reinforcement}
%Competitor networks can also retrain based on reinforcement learning. \textit{Forza Car Racing}'s "Drivatar" system is an excellent example. The \textit{Forza Racing} series is a long-running driving simulation in which the player accumulates money and renowned by winning increasingly difficult street and circuit races. Here, the neural network is being utilized to control all the NPC cars. While the player directly competes against the neural network, it retrains independently of the player, as it's reinforcement score stems from where it places in the race. The game does not make the player aware that the AI behind the NPC drivers is a neural network, and in fact isn't even made aware that the neural network is retraining and "getting better" as time goes on.



%\subsubsection{Reinforcement}
%\textit{GAR} is an excellent example of a \textit{designer} network that is based on a reinforcement architecture\todo{Seb: It's not RL but called interactive evolution. Maybe we should discuss this today}. In GAR, players pilot a spacecraft, to which you attach new weapons. These weapons are procedurally generated by the neural network. The neural network utilizes reinforcement learning to assign "scores" to various weapon attributes based on what weapons the player has used up to that point. Here, the interaction between network and player are indirect and hidden.

%\subsubsection{Player Input}
%More common, Designer neural networks operated based on player input. For example, \textit{AI Dungeon} designs plausible text adventures based on player inputted responses. In this instance, the player is directly interacting with the neural network; furthermore, the game goes out of its way to remind the player that the "Dungeon Master" in this experience is a neural network. 


%\subsubsection{Reinforcement}
%The dynamic teammate networks we encountered retrained via reinforcement learning. \textit{NERO} is a fascinating example, as it consists of two distinct gameplay phases, one of which is entirely based on training your neural networks. \textit{NERO} is a real-time strategy game, with an added twist that you do not directly control your units. Rather, you train your units before battle by having them focus on achieving a variety of goals--each goal trains the neural network to focus on a certain gameplay activity. In this case, the player is directly interacting with each neural network agent, and they are fully aware that what they're interacting with is a neural network.

%\subsubsection{Player Input}
 %make GAR clear - this is a unique case where they're pulling info from what the player has equipped so its a little more indirect.
% Teammate networks can also be static networks that render results based on player input. For example, \textit{Evolution} allows the player to give the neural network a few joints, bones, and muscles. The network then creates an animal/creature capable of locomotion based on the blueprint provided by the player. This collaborative effort to create a creature capable of a specific gameplay goal--such as walk or run a certain distance--is a great illustration of a network and player working hand in hand to achieve a shared gameplay goal. In this instance, the player isn't made explicitly aware that a neural network is at work behind the scenes.

==> prev_submission/archieved_docs/rushold.tex <==
%OLD SECTION 4.2
%Archived just in case we want to pull chunks of the writing out later.

%Within Online Learning NNs, we found that some outputted \textit{Content}. Here we see the NN supporting the player by providing them content that is both procedurally generated but also tailored to the individual player. A example of an Online Content NN is \textit{Petalz}. In this game, the flower is the product of the NN's output.

\subsubsection{Rewards}
Online reward input refers to a gamified version of reinforcement learning. This structure applies a value to every player action/outcome for a given activity and incentives the neural network to reproduce actions associated with higher point values for the action. For example... (add).

(Add number, percentage, and the types that occurred)

\subsubsection{Preferences}
Online preference input is where the NN learns from the player based on their gameplay preferences. These preferences can be actively or passively conveyed to the neural network. For example... (add)

(Add number, percentage, and the types that occurred)

\subsection{Offline Learning}
Offline learning NNs do not undergo retraining after interacting with individual players. These NNs are defined by their static nature; their function in regard to the player isn't concerned with learning about individuals, but rather providing an identical process to all players. For example... (add).

Of the 20 games, five games (25\%) were categorized as Offline Learning. These static neural networks can be further subdivided in two ways: 1) based on the type of output they render for the player and 2) what kind of input is expected from the player. 

\subsubsection{Content}
Neural networks can also output content for the player. This content might be the focus of the game, such as generating content for the player to experience or it might be a tertiary gameplay experience like dynamic background music generation. For example... (add).

(Add number, percentage, and the types that occurred)

\subsubsection{Behaviors}
Neural networks often output a behavioral decision for the agent they control. For offline learning, the NN... For example... (add).

\subsection{Offline Player Input}
Offline player input refers to NN that... (add description).

\subsubsection{Rewards}
Offline reward input refers to a gamified version of reinforcement learning. This structure applies a value to every player action/outcome for a given activity and incentives the neural network to reproduce actions associated with higher point values for the action. For example... (add).

\subsubsection{Preferences}
Offline preference input is where the NN... (description) For example... (add)

\subsubsection{Natural Language/Text}
Natural Language input is where the player uses open-ended text or spoken-language as the primary input to the neural network. For example... (add)

\subsubsection{Image}
Image input is where the player uses an open-ended image as the primary input to the neural network. For example...

%-------------- Previous draft. Comment out when done with the new format above --------%
%%%%%%%%%%%%%%%%%%%%

\subsubsection{Online Learning}
Online Learning NNs are retrained or tuned while or immediately after interacting with the player. Based on our analysis, fifteen games were categorized as using online learning. These NNs interact with the player, learning more about their tendencies, preferences, and/or strategies. Here the NNs bolster and/or simulate the player's belief that the game is evolving alongside them. Within this categorization, we found these Online NNs had two output methods, \textit{Behaviors} and \textit{Content}.

Behavior NNs output a decision or action for an NN-controlled agent from a limited list of pre-defined choices. For the player, this simulates artificial intelligence, as they watch NN-controlled game agent's act autonomously. The \textbf{Forza Series} \cite{takahashi_2018} is an example of an Online Behavior NN that outputs a behavior. The \textit{Forza} series is a well known car racing simulator. Its "Drivatar" system is a neural network that controls each NPC driver the player races against. This neural network continually retrains itself on a player's local machine and outputs driver behaviors. This adaptive behavior creates an opportunity for the neural network to exploit players that are over-reliant on a single strategy, therefore, creating an evolving challenge. While all of these NNs evolve alongside the individual player, there are some differentiating factors within this category. Namely, we observed two player input methods and two NN output methods.

Within Online Learning NNs, we found that some outputted \textit{Content}. Here we see the NN supporting the player by providing them content that is both procedurally generated but also tailored to the individual player. A example of an Online Content NN is \textit{Petalz}. In this game, the flower is the product of the NN's output. %Since we're at the length limit and we already described the gameplay of Petalz above, should we just mention it as an example and move on? Or at the least skip re-introducing the basic gameplay?

We also observed two player input methods used within  Online Learning, \textit{Rewards} and \textit{Preferences}. We found that seven games used a Reward input. This input method implements a gamified version of reinforcement learning, allowing for players to instruct the NN through rewards and punishments. For the player, this format bolsters the experience of "teaching" the NN with direct impact. For example, \textit{Creatures} \cite{grand1997creatures} accomplishes this through the player teaching the NN via reinforcement. The creature will perform different actions stochastically, and the player can increase or decrease the chances of the creature doing that specific action again by using the pet or slap game mechanic slapping.

%Within this online learning category, we found two of our four player-input methods present: \textit{Rewards} and \texit{Preferences}. 

%Rewards: Seven games retrained their networks with a reward-based input structure. For example, \textit{Creatures} is a tamogachi-style pet simulator. Like \textit{Black and White}, the neural network controls the actions of the player's pet, rather than the player having direct control. This network also retrains as it interacts with the player depending on whether the player slaps or strokes their pet after any given action. This allows the player to shape the network's behavior over time, allowing for a sense of educating on behalf of the player.

Second, we found that four games used a player's preference as its primary input. Whether actively chosen by the player or obtained via analyzing gameplay performance, these preferences directly impact the NNs results and thus the gameplay experience as a whole. For example, \textit{NERO} \cite{stanley2005evolving} is a game in which the player trains robot fighters by providing various roles for the robots to specialize. After training their robots, players pit their army against one another to see whose robots are better suited to complete the objective. Each player's robot is controlled by an individual NN, each learning different tactics based on the player's choices. The training phase allows the player's preferences to impact the NN and specialize their robots' fight strategies.


%Cut for space considerations for now, please dont delete yet tho in case we decide to use later.
%We also found two distinct output formats, \texit{Behaviors} and \textit{Content}. Behavior NNs output behavioral decisions from a limited set of options. Building on a previous example, the NN in \textit{Creatures} is constantly outputting behavioral decisions and actions for the creature to partake in. The player can augment the NN's behavior making via reinforcement, but the network always outputs a new behavior. In all of these examples, these behaviors are from a preset list of options, rather than true open-ended behavioral. In addition to Behavioral NNs, we also identified Online Content NNs.

%Online Content creators all provide procedurally generated content for the player. For example, \textit{GAR} is a spaceship-shooter in which new weapon spray patterns are procedurally generated. These NNs evolve in conjunction with the player; in \textit{GAR}'s case, the NN observes what spray patterns the player uses the most and creates new spray patterns based on that assumed preference. This slow process of learning the player's preferences leads to procedurally generated content that is tailor-made for individual players.



%\texit{Machine Learning Arena}. In \texit{Machine Learning Arena}, players train a NN to win a boxing match. They do so by boxing NPC opponents while the NN observes the player. After each match, the NN retrains on the new data, becoming a better boxer in the process. The player can then allow his NN-controlled trainee to fight the NPC. While all online NNs retrain, there were some differentiating factors among these NNs.

%Online Learning: Eleven games in our survey were categorized as online learning. Online learning refers to neural network retrains on new data after interacting with individual players. In all observed cases, this was used to learn more about individual player's tendencies and tactics. Furthermore, each game in this category has a network that outputs a \textit{Behavior}; no content-creation networks were observed in Online Learning. 

%We observed two categories for the NN's output in relation to the player. First, we observed NNs being used to create a custom set of game behaviors for the player to interact with, which is derived from the players' behavior inside the game. The game would learn about the players' tendencies and adapt to the game's behavior accordingly. For example, in the game series \textit{Forza}, their "Drivatar" system is a neural network that controls each driver. This neural network continually retrains itself on a player's local machine and outputs driver behaviors. This adaptive behavior creates an opportunity for the neural network to exploit players that are over-reliant on a single strategy, therefore, creating an evolving challenge. 
%We saw that there were two main reasons an Online network was chosen, in relation to the player: 1) a diverse set of options for player behavior, meaning the neural network is capable of learning individual player tendencies amongst a diverse set of options, or 2) because the player and the neural network were designed to grow in conjunction with one another.

%An example of the former type of design space is the "Drivatar" system in \textit{Forza Racing}. The \textit{Forza} series is a racing simulation game, and their "Drivatar" system is a neural network that controls each NPC racer. This neural network continually retrains itself on a player's local machine and is constantly outputting the decisions for the NPC racers. This works well in \textit{Forza} because there are a diverse set of player tactics--from aggressive racing to drafting behind other racers until the last moment. This diverse set of strategies means the neural network can adapt to and exploit players that are over reliant on a single strategy.

%Second, we also observed the NNs being used to grow in conjunction with the player. As opposed to the previous description, the difference is that the neural network is not just observing and providing an output, but rather, develops overtime based on the players preferences. For example, in the game \textit{Black and White}, players interact with a creature who is a neural network-controlled deity. The deity resides on an island that includes villagers, and can interact with a variety of objects in a variety of ways. The player has the option to reinforce the creatures behaviors and actions. This reinforcement can be positive or negative, making it possible to create a benevolent or malevolent deity by simply petting or slapping to shape its future behavior. %Can expand further if needed with examples of reinforcing to create an evil deity vs a good one 

%As for players and networks that grow together, \textit{Black & White} stands as a great example. In \textit{Black and White}, players interact with a neural network-controlled deity. The deity resides on an island that includes villagers, and can interact with a variety of objects in a variety of ways. The player has the option to reinforce the creatures behaviors and actions. This reinforcement can be positive or negative, making it possible to create a benevolent or malevolent deity by simply petting or slapping to shape its future behavior. %Can expand further if needed with examples of reinforcing to create an evil deity vs a good one 

%Preferences: Four games use a neural network that takes the player's preferences as an input. These networks "learn" each individual player's preferences by retraining after interacting with the player. For example, \textit{NERO} is a game in which the player trains robot fighters by giving them various tasks to specialize their training in, and then pits their fighters against another player's. Here, each robot is controlled by an individual neural network, each learning slightly differently based on the player's decisions. This allows the player to battle in his preferred way by allowing them to specialize their fighters as they see fit.
%Move to Discussion Section
%This structure works best for two different game designs: Pet Simulators where the designer wants the pet to demonstrate independence but ultimately subservience to the player, and zero-sum competitions in which identifying a winner and a loser is simple.   

%For example, \textit{Audio in Space} is a spaceship-shooter in which the player must avoid large rocks and use their weapons to destroy smaller rocks. Here, two separate neural networks work in conjunction to create unique weapon-spray patterns and background music procedurally. The players get to experience unique, but tailored, procedural content without hazarding true randomness. 

\subsubsection{Offline Learning}    
Offline learning NNs do not undergo retraining after interacting with individual players. These NNs are defined by their static nature; their function in regard to the player isn't concerned with learning about individuals, but rather providing an identical process to all players. Five games were categorized as Offline Learning. These static neural networks can be further subdivided in two ways: 1) based on the type of output they render for the player and 2) what kind of input is expected from the player.   %In general, these networks are more interested in treating all players as a monolith rather than as individuals.

In terms of output, we discovered the same two categories within Offline learners: \textit{Content} and \texit{Behavior}. Content NNs take the form of PCGs. That is, their output is various forms of game content to help diversify the player's gameplay experience without overburdening developers with asset creation. For example, \textit{Darwin's Avatar} \cite{lessin2015darwin} is a game in which players attempt to ambulate a PCG creature constructed through an evolutionary process. These creatures are generated and a neural network outputs control signals for each muscle, and is trained alongside the creature's evolution. Once a certain fitness threshold is met, the NN control is removed and the player attempts to control the creature. Here we can see that the network does not learn, evolve, or grow alongside the player, but rather treats all players the same. This type of output is associated with only one input method: \textit{Preferences}.

In addition to Content, we also identified four Offline NNs that output \texit{Behaviors}. While these games were in the minority, they share a lot of commonalities. Here, the NNs consistency among all of the players is key for the game to function properly. v

%This paragraph might be out of scope/can be on cutting block/moved to discussion sec.
These Offline Learning networks that render Behaviors all utilize advanced neural networks that were trained outside the scope of the game. This design space tends to implement a neural network far more advanced than normal gaming neural networks by incorporating a preexisting network in the foundation of the game design. If designers are looking to implement the strongest pretrained neural networks available, this is the route to follow.
    
These Offline Behavior NNs receive input from the player in one of two ways: through natural language and text, or through images. Here the NNs support players' open-ended input appropriately, opening up new gameplay avenues. Three games used language and text as their input. For example, \textit{Semantris} \cite{semantris} is a game in which the player must type a word that will correlate most strongly to one highlighted word from a list of ten. Here, the player is interacting with an advanced neural network under the guise of a game. This allows the player-network interaction to be more dynamic and responsive than networks designed within the scope of a game. Another input option for Offline Behavior NNs is images.
    
    %This game was built with a neural network that trained to be able to predict how likely one statement would follow another as a response. Like its peer \textit{Hey Robot} these unsupervised neural networks output a decision for the player. 
Google's \textit{Quick, Draw!} \cite{quick} is based around a neural network trained on millions of hand-drawn sketches, each labelled with a proper categorization. The neural network then receives new, unlabelled data from players and categorizes the sketch with one of the labels it was exposed to during training. Like \textit{Semantris}, the hook for the player is more the robust and accurate neural network, rather than the minimum gameplay mechanics that were designed around the network.


% OLD DISCUSSION
\emph{NN replacing existing game mechanics.} A common theme we observed when analyzing how NN supported the player experience was that \glspl{ann} were used to replace common game mechanics usually developed by another AI approaches\todo{Mat: 'another AI approaches? Should it be human instead? Or is it other AI/ML algorithmic approaches}. This trend was most prevalent in \glspl{ann} as competitors and designers.

In \gls{ann} as competitor, we see a commonality in the \gls{ann} replacing traditional decision trees. \glspl{ann} allows the developers to detangle \gls{ai} logic and condense that part of the codebase significantly rather than have to code out every conceivable scenario and an appropriate reaction. In an industry where small teams need to be efficient as possible, and larger ones are plagued by "crunch," it seems vital to be as concise as possible when creating new code \todo{Mat: isn't it more due to the fact that you cannot create code for every conceivable scenario so you HAVE to use some better, more general, decision logic. With the large number of dimensions for any interesting problem it would be impossible to cover by hand - even for a large team of developers}. 
%
A possible direction for further study would be investigating the effectiveness of this substitution. Studying whether or not \gls{ann}-controlled agents significantly outperform \todo{Are we comparing the NN to handcrafted decision trees? Because decision trees can also be generated and considered part of AI, so this will have to be clarified.} decision-tree agents would give assurance to other developers that the time investment of implementing a new system will be a benefit in the long run. Even more interesting would be to investigate whether developers that have made the switch did so with data supporting the decision. Lastly, investigating whether or not players enjoy this experience more than previous \gls{ai} options is another important factor, as more work is needed to understand where the intersection of player and developer preferences are when it comes to replacing enemy \gls{ai} with \glspl{ann}. 

In \gls{ann} as designer, we observed a similar phenomenon in which their inclusion replaces what was previously a time-consuming aspect of development: asset creation. \glspl{ann} help circumvents this bottleneck by handing off at least some of the asset-creation process. This can be especially helpful when development teams are engineer-heavy and cannot overburden artists by asking for hundreds of variations of basic assets. We again see a situation where neither is inherently "better" or "worse", but rather very situation-dependent. Again, we see the importance of knowing all the tools available to a team to maximize their efficiency.

Similar areas of future study enter the picture as with competitor \glspl{ann}. Namely, investigating whether or not players enjoy PGC more than traditional forms. And building off of that, is there a certain scale that must be achieved in order to convince players that prefer traditional assets that PGC was worth implementing. This area of study would illuminate our understanding of human's appreciation of \gls{ai} art and give us a sense of what scale it takes to "wow" the average gamer with procedural content.

==> prev_submission/game_analysis_mainTable_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lccccccc}
\multicolumn{1}{c}{\textbf{Game Title, Ludography}} & \textbf{Developer} & \textbf{Genre} & \textbf{Interaction Metaphor} & \textbf{UI Visibility} & \textbf{NN Input} & \textbf{NN Output} & \textbf{Online/Offline Learning} \\
\rowcolor[HTML]{EFEFEF} 
AI Dungeon {\citeL{aidungeon}}                                & Indie              & Adventure      & NN as Designer                & NN-Limited          & Natural Language  & Behaviors          & Offline                          \\
Aivolution {\citeL{aivolution}}                                & Indie              & Simulation     & NN as Teammate                & NN-Limited          & Preference        & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
AudioinSpace* {\citeL{hoover2015audioinspace}\cite{audioinspace:hoover2015audioinspace}}                             & Research           & Action         & NN as Designer                & NN-Agnostic         & Preference        & Content            & Online                           \\
Black \& White {\citeL{blackandwhite}\cite{blackandwhite:wexler2002artificial}}                            & AAA                & Role-play      & NN as Apprentice              & NN-Agnostic         & Rewards           & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
Blitzkrieg 3 {\citeL{blitzkrieg}}                              & AAA                & Strategy       & NN as Competitor              & NN-Limited          & Preference        & Behaviors          & Offline                          \\
BrainCrafter * {\cite{braincrafter}}                            & Research           & Puzzle         & NN as Apprentice              & NN-Specific          & Preference        & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
Corral {\citeL{corral}}                                    & Indie              & Simulation     & NN as Apprentice              & NN-Agnostic         & Preference        & Behaviors          & Online                           \\
Creatures {\cite{grand1997creatures}\cite{creatures:grand1997creatures}}                                 & AAA                & Role-play      & NN as Apprentice              & NN-Agnostic         & Rewards           & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
Darwin's Avatars * {\citeL{lessin2015darwin} \cite{darwinsavatar:lessin2015darwin}}                         & Research           & Action         & NN as Designer                & NN-Limited          & Preference        & Content            & Offline                          \\
Democracy 3 {\citeL{democracy}}                              & AAA                & Role-play      & NN as Designer                & NN-Agnostic         & Preference        & Behaviors          & Offline                          \\
\rowcolor[HTML]{EFEFEF} 
Dr. Derk's Mutant Battlegrounds {\citeL{derks}}           & Indie              & Simulation     & NN as Apprentice              & NN-Limited          & Rewards           & Behaviors          & Online                           \\
EvoCommander * {\citeL{jallov2016evocommander} \cite{evocommander:jallov2016evocommander}}                            & Research           & Simulation     & NN as Apprentice              & NN-Specific          & Preference        & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
Evolution {\citeL{evolution}}                                  & Indie              & Simulation     & NN as Teammate                & NN-Specific          & Preference        & Behaviors          & Online                           \\
evolution for beginners {\citeL{evolutionbeg}}                   & Indie              & Simulation     & NN as Apprentice              & NN-Limited          & Preference        & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
Football Evo {\citeL{football}}                               & Indie              & Simulation     & NN as Apprentice              & NN-Limited          & Rewards           & Behaviors          & Online                           \\
Forza Car Racing {\citeL{forza}\cite{forza:takahashi_2018}}                           & AAA                & Sports         & NN as Competitor              & NN-Limited          & Rewards           & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
GAR {\cite{hastings2009evolving}\cite{gar:hastings2009evolving}}                                       & Research           & Action         & NN as Designer                & NN-Limited          & Preference        & Content            & Online                           \\
Gridworld {\citeL{grid}}                                  & Indie              & Simulation     & NN as Designer                & NN-Limited          & Preference        & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
Guess the Word \citeL{guesstheword}  \cite{guesstheword:publication}                           & Research           & Puzzle         & NN as Teammate                & NN-Limited          & Natural Language  & Behaviors          & Offline                          \\
Hey Robot {\citeL{hey}}                                 & Indie              & Puzzle         & NN as Teammate                & NN-Agnostic         & Natural Language  & Behaviors          & Offline                          \\
\rowcolor[HTML]{EFEFEF} 
How to Train your Snake {\citeL{snake}}                    & Indie              & Simulation     & NN as Apprentice              & NN-Specific          & Rewards           & Behaviors          & Online                           \\
Idle Machine Learning Game {\citeL{idle}}                & Indie              & Simulation     & NN as Apprentice              & NN-Specific          & Rewards           & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
iNNk {[}33{]}                                       & Research           & Puzzle         & NN as Competitor              & NN-Specific          & Image             & Behaviors          & Offline                          \\
Machine Learning Arena * {\citeL{ferguson2019machine}\cite{machinelearningarena:ferguson2019machine}}                   & Research           & Simulation     & NN as Teammate                & NN-Specific          & Rewards           & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
MotoGP19 {\citeL{moto}}                                  & AAA                & Sports         & NN as Competitor              & NN-Agnostic         & Rewards           & Behaviors          & Offline                          \\
Neat Race {\citeL{neat}}                                 & Indie              & Simulation     & NN as Apprentice              & NN-Specific          & Rewards           & Behaviors          & Online                           \\
\rowcolor[HTML]{EFEFEF} 
NERO {\citeL{stanley2005evolving}\cite{nero:stanley2005evolving}}                                      & Research           & Simulation     & NN as Apprentice              & NN-Specific          & Preference        & Behaviors          & Online                           \\
Petalz* {\citeL{risi2015petalz}\cite{petalzpublication:risi2015petalz}}                                   & Research           & Simulation     & NN as Designer                & NN-Agnostic         & Preference        & Content            & Offline                          \\
\rowcolor[HTML]{EFEFEF} 
Quick, Draw! {\citeL{quick}}                              & Research           & Puzzle         & NN as Teammate                & NN-Limited          & Image             & Behaviors          & Offline                          \\
Race for the Galaxy {\citeL{raceforthegalaxy}}                        & AAA                & Strategy       & NN as Competitor              & NN-Limited          & Preference        & Behaviors          & Offline                          \\
\rowcolor[HTML]{EFEFEF} 
Roll for the Galaxy {\citeL{rollforthegalaxy}}                                 & AAA                & Strategy       & NN as Competitor              & NN-Limited          & Preference        & Behaviors          & Offline                          \\
Semantris {\citeL{semantris}}                                 & Research           & Puzzle         & NN as Teammate                & NN-Limited          & Natural Language  & Behaviors          & Offline                          \\
\rowcolor[HTML]{EFEFEF} 
Supreme Commander 2 {\citeL{rabin2015game}\cite{supremecommander:rabin2015game}}                       & AAA                & Strategy       & NN as Competitor              & NN-Agnostic         & Preference        & Behaviors          & Offline                          \\
The Abbattoir Intergrade {\citeL{abbattoir}}                   & Indie              & Strategy       & NN as Competitor              & NN-Agnostic         & Preference        & Behaviors          & Online                     
\end{tabular}
\end{adjustbox}
\caption{Results of player-AI interaction in NN games }
%\label{tab:game_analysis_mainTable} 
\end{table*}

==> tables/game_analysis_mainTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \rotatebox{90}{
\begin{sidewaystable*}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{p{4cm}ccp{2cm}ccccp{1.5cm}p{5.3cm}}
\multicolumn{1}{c}{\textbf{Game Title [Ludography]}} & \textbf{Publisher}          & \textbf{Genre}                   & \textbf{Interaction Metaphor}            & \textbf{UI}                & \textbf{NN Input}                  & \textbf{NN Output}                & \textbf{Learning} & \textbf{Multiple AIs?}  & \multicolumn{1}{c}{\textbf{NN Responsibilties}}                    \\
\rowcolor[HTML]{F3F3F3} 
2D Walk Evolution {\citeL{2dwalkevolution}}                                   & Indie                       & Simulation                       & Teammate                           & NN-Specific                        & Preference                         & Behaviors                         & Offline                          & No                              & NN controls creature movement.                                     \\
AI Dungeon {\citeL{aidungeon}}                                           & Indie                       & Adventure                        & Designer                           & NN-Limited                         & Natural Language                   & Behaviors                         & Offline                          & No                              & NN creates natural language responses.                             \\
\rowcolor[HTML]{F3F3F3} 
Aivolution {\citeL{aivolution}}                                          & Indie                       & Simulation                       & Teammate                           & NN-Limited                         & Preference                         & Behaviors                         & Online                           & Unknown                         & NN controls creature movement.                                     \\
AudioinSpace* {\citeL{hoover2015audioinspace}\cite{audioinspace:hoover2015audioinspace}}                                      & Research                    & Action                           & Designer                           & NN-Agnostic                        & Preference                         & Content                           & Online                           & Yes                             & NN creates weapon visuals and audio.                               \\
\rowcolor[HTML]{F3F3F3} 
Black \& White {\citeL{blackandwhite}\cite{blackandwhite:wexler2002artificial}}                                      & AAA                         & Role-play                        & Apprentice                         & NN-Agnostic                        & Rewards                            & Behaviors                         & Online                           & Yes                             & NN creates creature desires.                                       \\
Blitzkrieg 3 {\citeL{blitzkrieg}}                                        & AAA                         & Strategy                         & Competitor                         & NN-Limited                         & Preference                         & Behaviors                         & Offline                          & Unknown                         & NN controls "Boris" battle behavior.                               \\
\rowcolor[HTML]{F3F3F3} 
BrainCrafter * {\cite{braincrafter}}                                     & Research                    & Puzzle                           & Apprentice                         & NN-Specific                        & Preference                         & Behaviors                         & Online                           & No                              & NN controls robot movement.                                        \\
Colin McRae Rally 2.0* {\citeL{colin}}                             & AAA                         & Sports                           & Competitor                         & NN-Agnostic                        & Rewards                            & Behaviors                         & Offline                          & Unknown                         & \cellcolor[HTML]{F3F3F3}NN controls the car's driving performance. \\
\rowcolor[HTML]{F3F3F3} 
Competitive Snake {\citeL{competitivesnake}}                                  & Indie                       & Puzzle                           & Competitor                         & NN-Agnostic                        & Rewards                            & Behaviors                         & Offline                          & No                              & NN controls enemy snake behavior.                                  \\
Corral {\citeL{corral}}                                              & Indie                       & Simulation                       & Apprentice                         & NN-Agnostic                        & Preference                         & Behaviors                         & Online                           & Unknown                         & NN controls chicken movement and preservation skills.              \\
\rowcolor[HTML]{F3F3F3} 
Creatures {\cite{grand1997creatures}\cite{creatures:grand1997creatures}}                                           & AAA                         & Role-play                        & Apprentice                         & NN-Agnostic                        & Rewards                            & Behaviors                         & Online                           & Yes                             & NN controls the creature's sensor-motor coordination.              \\
Darwin's Avatar* {\citeL{lessin2015darwin} \cite{darwinsavatar:lessin2015darwin}}                                   & Research                    & Action                           & Designer                           & NN-Limited                         & Preference                         & Content                           & Offline                          & No                              & NN controls creature movement.                                     \\
\rowcolor[HTML]{F3F3F3} 
Democracy 3 {\citeL{democracy}}                                         & AAA                         & Role-play                        & Designer                           & NN-Agnostic                        & Preference                         & Behaviors                         & Offline                          & Unknown                         & NN creates motivations and desires of the public.                  \\
Dr. Derk's Mutant Battlegrounds {\citeL{derks}}                     & Indie                       & Simulation                       & Apprentice                         & NN-Limited                         & Rewards                            & Behaviors                         & Online                           & Unknown                         & NN controls creature movement and behavior.                        \\
\rowcolor[HTML]{F3F3F3} 
EvoCommander* {\citeL{jallov2016evocommander} \cite{evocommander:jallov2016evocommander}}                                      & Research                    & Simulation                       & Apprentice                         & NN-Specific                        & Preference                         & Behaviors                         & Online                           & No                              & NN controls tank movement and shooting behavior.                   \\
Evolution {\citeL{evolution}}                                           & Indie                       & Simulation                       & Teammate                           & NN-Specific                        & Preference                         & Behaviors                         & Online                           & Unknown                         & NN controls creature movement.                                     \\
\rowcolor[HTML]{F3F3F3} 
evolution for beginners {\citeL{evolutionbeg}}                             & Indie                       & Simulation                       & Apprentice                         & NN-Limited                         & Preference                         & Behaviors                         & Online                           & Unknown                         & NN controls creature movement and sensory input.                   \\
Football Evo {\citeL{football}}                                        & Indie                       & Simulation                       & Apprentice                         & NN-Limited                         & Rewards                            & Behaviors                         & Online                           & No                              & NN controls player movement and behavior.                          \\
\rowcolor[HTML]{F3F3F3} 
Forza Car Racing {\citeL{forza}\cite{forza:takahashi_2018}}                                   & AAA                         & Sports                           & Competitor                         & NN-Limited                         & Rewards                            & Behaviors                         & Online                           & Unknown                         & NN controls the car's driving performance.                         \\
GAR {\cite{hastings2009evolving}\cite{gar:hastings2009evolving}}                                                 & Research                    & Action                           & Designer                           & NN-Limited                         & Preference                         & Content                           & Online                           & Yes                             & NN creates particle weapons.                                       \\
\rowcolor[HTML]{F3F3F3} 
Gridworld {\citeL{grid}}                                          & Indie                       & Simulation                       & Designer                           & NN-Limited                         & Preference                         & Behaviors                         & Online                           & Unknown                         & NN controls creature behavior.                                     \\
Guess the Word \citeL{guesstheword}  \cite{guesstheword:publication}                                     & Research                    & Puzzle                           & Teammate                           & NN-Limited                         & Natural Language                   & Behaviors                         & Offline                          & Yes                             & NN creates natural language responses.                             \\
\rowcolor[HTML]{F3F3F3} 
Hey Robot {\citeL{hey}}                                          & Indie                       & Puzzle                           & Teammate                           & NN-Agnostic                        & Natural Language                   & Behaviors                         & Offline                          & No                              & NN controls language processing.                                   \\
How to Train your Snake {\citeL{snake}}                            & Indie                       & Simulation                       & Apprentice                         & NN-Specific                        & Rewards                            & Behaviors                         & Online                           & No                              & NN controls snake movement.                                        \\
\rowcolor[HTML]{F3F3F3} 
Idle Machine Learning Game {\citeL{idle}}                         & Indie                       & Simulation                       & Apprentice                         & NN-Specific                        & Rewards                            & Behaviors                         & Online                           & No                              & NN controls performance of the vehicle's movement.                 \\
iNNk {\citeL{villareale2020innk}}                                              & Research                    & Puzzle                           & Competitor                         & NN-Specific                        & Image                              & Behaviors                         & Offline                          & No                              & NN identifies sketches drawn by the player.                        \\
\rowcolor[HTML]{F3F3F3} 
Machine Learning Arena *                            & Research                    & Simulation                       & Teammate                           & NN-Specific                        & Rewards                            & Behaviors                         & Online                           & Unknown                         & NN controls robot behavior.                                        \\
MotoGP19 {\citeL{moto}}                                           & AAA                         & Sports                           & Competitor                         & NN-Agnostic                        & Rewards                            & Behaviors                         & Offline                          & Unknown                         & NN controls the car's driving performance.                         \\
\rowcolor[HTML]{F3F3F3} 
Neat Race {\citeL{neat}}                                          & Indie                       & Simulation                       & Apprentice                         & NN-Specific                        & Rewards                            & Behaviors                         & Online                           & No                              & NN controls car movement.                                          \\
NERO {\citeL{stanley2005evolving}\cite{nero:stanley2005evolving}}                                               & Research                    & Simulation                       & Apprentice                         & NN-Specific                        & Preference                         & Behaviors                         & Online                           & No                              & NN controls robot movement and shooting behavior.                  \\
\rowcolor[HTML]{F3F3F3} 
Oui Chef!! {\citeL{oui}\cite{cimolino2019oui}}                                         & Research                    & Role-play                        & Apprentice                         & NN-Agnostic                        & Preference                         & Behaviors                         & Online                           & No                              & NN controls chef behavior.                                         \\
Petalz* {\citeL{risi2015petalz}\cite{petalzpublication:risi2015petalz}}                                            & Research                    & Simulation                       & Designer                           & NN-Agnostic                        & Preference                         & Content                           & Offline                          & No                              & NN creates flowers.                                                \\
\rowcolor[HTML]{F3F3F3} 
Quick, Draw! {\citeL{quick}}                                       & Research                    & Puzzle                           & Teammate                           & NN-Limited                         & Image                              & Behaviors                         & Offline                          & No                              & NN identifies sketches drawn by the player.                        \\
Race for the Galaxy {\citeL{raceforthegalaxy}}                                & AAA                         & Strategy                         & Competitor                         & NN-Limited                         & Preference                         & Behaviors                         & Offline                          & Unknown                         & NN controls opponent behavior.                                     \\
\cellcolor[HTML]{F3F3F3}Roll for the Galaxy {\citeL{rollforthegalaxy}}         & \cellcolor[HTML]{F3F3F3}AAA & \cellcolor[HTML]{F3F3F3}Strategy & \cellcolor[HTML]{F3F3F3}Competitor & \cellcolor[HTML]{F3F3F3}NN-Limited & \cellcolor[HTML]{F3F3F3}Preference & \cellcolor[HTML]{F3F3F3}Behaviors & \cellcolor[HTML]{F3F3F3}Offline  & \cellcolor[HTML]{F3F3F3}Unknown & NN controls opponent behavior.                                     \\
Semantris {\citeL{semantris}}                                          & Research                    & Puzzle                           & Teammate                           & NN-Limited                         & Natural Language                   & Behaviors                         & Offline                          & No                              & NN controls the classification of words.                           \\
\rowcolor[HTML]{F3F3F3} 
Supreme Commander 2 {\citeL{rabin2015game}\cite{supremecommander:rabin2015game}}                                & AAA                         & Strategy                         & Competitor                         & NN-Agnostic                        & Preference                         & Behaviors                         & Offline                          & Yes                             & NN controls enemy unit flight and fight behavior.                  \\
The Abbattoir Intergrade {\citeL{abbattoir}}                            & Indie                       & Strategy                         & Competitor                         & NN-Agnostic                        & Preference                         & Behaviors                         & Online                           & Unknown                         & NN controls enemy unit offense behavior.                          
\end{tabular}
\end{adjustbox}
\caption{Results of player-AI interaction in NN games. \changed{Games marked with * do not have playable versions publicly available. These games are excluded for Phase 2.} {\color{red}What does the * mean. Add the info here so that the table is self-contained. Is evolution for beginners intentionally in lower-cases?}}
\label{tab:game_analysis_mainTable} 
\end{sidewaystable*}
% }

==> tables/game_analysis_mainTable2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{sidewaystable*}
\caption{Results of player-AI interaction in NN games. \changed{Games marked with * do not have playable versions publicly available. These games are excluded for Phase 2.} {\color{red}What does the * mean. Add the info here so that the table is self-contained. Is evolution for beginners intentionally in lower-cases?}}
\label{tab:game_analysis_mainTable}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{lcccccccl}
\multicolumn{1}{l}{\textbf{Game Title {[}Ludography{]}}} & \textbf{Publisher}          & \textbf{Genre}                   & \textbf{Interaction Metaphor}      & \textbf{UI}                           & \textbf{NN Output}                & \textbf{Learning}               & \textbf{Multiple AIs?}          & \multicolumn{1}{c}{\textbf{NN Responsibilities}}               \\
\rowcolor[HTML]{F3F3F3} 
2D Walk Evolution {\citeL{2dwalkevolution}}                                       & Indie                       & Simulation                       & Teammate                           & NN-Specific                           & Behaviors                         & Offline                         & No                              & controls creature movement                                     \\
AI Dungeon {\citeL{aidungeon}}                                               & Indie                       & Adventure                        & Designer                           & NN-Limited                            & Behaviors                         & Offline                         & No                              & creates natural language responses                             \\
\rowcolor[HTML]{F3F3F3} 
Aivolution {\citeL{aivolution}}                                                & Indie                       & Simulation                       & Teammate                           & NN-Limited                            & Behaviors                         & Online                          & Unknown                         & controls creature movement                                     \\
AudioinSpace* {\citeL{hoover2015audioinspace}\cite{audioinspace:hoover2015audioinspace}}                                           & Research                    & Action                           & Designer                           & NN-Agnostic                           & Content                           & Online                          & Yes                             & creates weapon visuals and audio                               \\
\rowcolor[HTML]{F3F3F3} 
Black \& White {\citeL{blackandwhite}\cite{blackandwhite:wexler2002artificial}}                                          & AAA                         & Role-play                        & Apprentice                         & NN-Agnostic UI                        & Behaviors                         & Online                          & Yes                             & creates creature desires                                       \\
Blitzkrieg 3 {\citeL{blitzkrieg}}                                            & AAA                         & Strategy                         & Competitor                         & NN-Limited UI                         & Behaviors                         & Offline                         & Unknown                         & controls "Boris" battle behavior                               \\
\rowcolor[HTML]{F3F3F3} 
BrainCrafter* {\cite{braincrafter}}                                          & Research                    & Puzzle                           & Apprentice                         & NN-Specific UI                        & Behaviors                         & Online                          & No                              & controls robot movement                                        \\
Colin McRae Rally 2.0* {\citeL{colin}}                                  & AAA                         & Sports                           & Competitor                         & NN-Agnostic UI                        & Behaviors                         & Offline                         & Unknown                         & \cellcolor[HTML]{F3F3F3}controls the car's driving performance \\
\rowcolor[HTML]{F3F3F3} 
Competitive Snake {\citeL{competitivesnake}}                                       & Indie                       & Puzzle                           & Competitor                         & NN-Agnostic UI                        & Behaviors                         & Offline                         & No                              & controls enemy snake behavior                                  \\
Corral {\citeL{corral}}                                                  & Indie                       & Simulation                       & Apprentice                         & NN-Agnostic UI                        & Behaviors                         & Online                          & Unknown                         & controls chicken movement and preservation skills              \\
\rowcolor[HTML]{F3F3F3} 
Creatures {\cite{grand1997creatures}\cite{creatures:grand1997creatures}}                                               & AAA                         & Role-play                        & Apprentice                         & NN-Agnostic UI                        & Behaviors                         & Online                          & Yes                             & controls the creature's sensor-motor coordination              \\
Darwin's Avatar* {\citeL{lessin2015darwin} \cite{darwinsavatar:lessin2015darwin}}                                       & Research                    & Action                           & Designer                           & NN-Limited UI                         & Content                           & Offline                         & No                              & controls creature movement                                     \\
\rowcolor[HTML]{F3F3F3} 
Democracy 3 {\citeL{democracy}}                                             & AAA                         & Role-play                        & Designer                           & NN-Agnostic UI                        & Behaviors                         & Offline                         & Unknown                         & creates motivations and desires of the public                  \\
Dr. Derk's Mutant Battlegrounds {\citeL{derks}}                         & Indie                       & Simulation                       & Apprentice                         & NN-Limited UI                         & Behaviors                         & Online                          & Unknown                         & controls creature movement and behavior                        \\
\rowcolor[HTML]{F3F3F3} 
EvoCommander* {\citeL{jallov2016evocommander} \cite{evocommander:jallov2016evocommander}}                                          & Research                    & Simulation                       & Apprentice                         & NN-Specific UI                        & Behaviors                         & Online                          & No                              & controls tank movement and shooting behavior                   \\
Evolution {\citeL{evolution}}                                               & Indie                       & Simulation                       & Teammate                           & NN-Specific UI                        & Behaviors                         & Online                          & Unknown                         & controls creature movement                                     \\
\rowcolor[HTML]{F3F3F3} 
evolution for beginners {\citeL{evolutionbeg}}                                 & Indie                       & Simulation                       & Apprentice                         & NN-Limited UI                         & Behaviors                         & Online                          & Unknown                         & controls creature movement and sensory input                   \\
Football Evo {\citeL{football}}                                            & Indie                       & Simulation                       & Apprentice                         & NN-Limited UI                         & Behaviors                         & Online                          & No                              & controls player movement and behavior                          \\
\rowcolor[HTML]{F3F3F3} 
Forza Car Racing {\citeL{forza}\cite{forza:takahashi_2018}}                                        & AAA                         & Sports                           & Competitor                         & NN-Limited UI                         & Behaviors                         & Online                          & Unknown                         & controls the car's driving performance                         \\
GAR {\cite{hastings2009evolving}\cite{gar:hastings2009evolving}}                                                     & Research                    & Action                           & Designer                           & NN-Limited UI                         & Content                           & Online                          & Yes                             & creates particle weapons                                       \\
\rowcolor[HTML]{F3F3F3} 
Gridworld {\citeL{grid}}                                              & Indie                       & Simulation                       & Designer                           & NN-Limited UI                         & Behaviors                         & Online                          & Unknown                         & controls creature behavior                                     \\
Guess the Word {\citeL{guesstheword}  \cite{guesstheword:publication}}                                          & Research                    & Puzzle                           & Teammate                           & NN-Limited UI                         & Behaviors                         & Offline                         & Yes                             & creates natural language responses                             \\
\rowcolor[HTML]{F3F3F3} 
Hey Robot {\citeL{hey}}                                               & Indie                       & Puzzle                           & Teammate                           & NN-Agnostic UI                        & Behaviors                         & Offline                         & No                              & controls language processing                                   \\
How to Train your Snake {\citeL{snake}}                                 & Indie                       & Simulation                       & Apprentice                         & NN-Specific UI                        & Behaviors                         & Online                          & No                              & controls snake movement                                        \\
\rowcolor[HTML]{F3F3F3} 
Idle Machine Learning Game {\citeL{idle}}                              & Indie                       & Simulation                       & Apprentice                         & NN-Specific UI                        & Behaviors                         & Online                          & No                              & controls performance of the vehicle's movement                 \\
iNNk {\citeL{villareale2020innk}}                                                    & Research                    & Puzzle                           & Competitor                         & NN-Specific UI                        & Behaviors                         & Offline                         & No                              & identifies sketches drawn by the player                        \\
\rowcolor[HTML]{F3F3F3} 
Machine Learning Arena* {\citeL{ferguson2019machine}}                                & Research                    & Simulation                       & Teammate                           & NN-Specific UI                        & Behaviors                         & Online                          & Unknown                         & controls robot behavior                                        \\
MotoGP19 {\citeL{moto}}                                                & AAA                         & Sports                           & Competitor                         & NN-Agnostic UI                        & Behaviors                         & Offline                         & Unknown                         & controls the car's driving performance                         \\
\rowcolor[HTML]{F3F3F3} 
Neat Race {\citeL{neat}}                                               & Indie                       & Simulation                       & Apprentice                         & NN-Specific UI                        & Behaviors                         & Online                          & No                              & controls car movement                                          \\
NERO {\citeL{stanley2005evolving}\cite{nero:stanley2005evolving}}                                                    & Research                    & Simulation                       & Apprentice                         & NN-Specific UI                        & Behaviors                         & Online                          & No                              & controls robot movement and shooting behavior                  \\
\rowcolor[HTML]{F3F3F3} 
Oui Chef!! {\citeL{oui}\cite{cimolino2019oui}}                                              & Research                    & Role-play                        & Apprentice                         & NN-Agnostic UI                        & Behaviors                         & Online                          & No                              & controls chef behavior                                         \\
Petalz* {\citeL{risi2015petalz}\cite{petalzpublication:risi2015petalz}}                                                 & Research                    & Simulation                       & Designer                           & NN-Agnostic UI                        & Content                           & Offline                         & No                              & creates flowers                                                \\
\rowcolor[HTML]{F3F3F3} 
Quick, Draw! {\citeL{quick}}                                            & Research                    & Puzzle                           & Teammate                           & NN-Limited UI                         & Behaviors                         & Offline                         & No                              & identifies sketches drawn by the player                        \\
Race for the Galaxy {\citeL{raceforthegalaxy}}                                     & AAA                         & Strategy                         & Competitor                         & NN-Limited UI                         & Behaviors                         & Offline                         & Unknown                         & controls opponent behavior                                     \\
\cellcolor[HTML]{F3F3F3}Roll for the Galaxy {\citeL{rollforthegalaxy}}             & \cellcolor[HTML]{F3F3F3}AAA & \cellcolor[HTML]{F3F3F3}Strategy & \cellcolor[HTML]{F3F3F3}Competitor & \cellcolor[HTML]{F3F3F3}NN-Limited UI & \cellcolor[HTML]{F3F3F3}Behaviors & \cellcolor[HTML]{F3F3F3}Offline & \cellcolor[HTML]{F3F3F3}Unknown & controls opponent behavior                                     \\
Semantris {\citeL{semantris}}                                               & Research                    & Puzzle                           & Teammate                           & NN-Limited UI                         & Behaviors                         & Offline                         & No                              & controls the classification of words                           \\
\rowcolor[HTML]{F3F3F3} 
Supreme Commander 2 {\citeL{rabin2015game}\cite{supremecommander:rabin2015game}}                                     & AAA                         & Strategy                         & Competitor                         & NN-Agnostic UI                        & Behaviors                         & Offline                         & Yes                             & controls enemy unit flight and fight behavior                  \\
The Abbattoir Intergrade {\citeL{abbattoir}}                                & Indie                       & Strategy                         & Competitor                         & NN-Agnostic UI                        & Behaviors                         & Online                          & Unknown                         & controls enemy unit offense behavior                          
\end{tabular}
\end{adjustbox}
\end{sidewaystable*}

==> tables/table-codes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\begin{tabular}{|c|p{80mm}|p{80mm}|}
\hline
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{AI Design Guidelines}}         & \multicolumn{1}{c|}{\textbf{Codes for Games}} \\ \hline
\multirow{6}{*}{Initially}               & \multirow{3}{=}{G1. Make clear what the system can do - Help the user understand what the AI system is capable of doing. } & G1A. Makes the NNs capabilities known
          \\ \cline{3-3} 
                                &                  & G1B. Makes part of NN’s capabilities known          \\ \cline{3-3} 
                                &                   & G1C. Does not make the capabilities known at all          \\ \cline{2-3} 
                                & \multirow{3}{=}{G2. Make clear how well the system can do what it can do - Help the user understand how often the AI system may make mistakes.} & G2A. Makes the NN’s limitations known           \\ \cline{3-3} 
                                &                   & G2B. Makes part of NN’s limitations known           \\ \cline{3-3} 
                                &                   & G2C. Does not make the limitations known at all          \\ \hline
\multirow{12}{*}{During}              & \multirow{3}{=}{G3. Timed services based on context - Time when to act or interrupt based on the user’s current task and environment.} & G3A. NN provides a timely service that adds to the flow of player experience.          \\ \cline{3-3} 
                                &                   & G3B. NN provides a timely service at the request of the player to continue the flow of player experience.\\ \cline{3-3} 
                                &                   & G3C. NN provides a timely service that interrupts the flow of player experience.          \\ \cline{2-3} 
                                & \multirow{3}{=}{G4. Show contextually relevant information - Display information relevant to the user’s current task and environment.} & G4A. Shows relevant feedback: UI + Behavior/content          \\ \cline{3-3} 
                                &                   & G4B. Shows some relevant feedback: behavior/content          \\ \cline{3-3} 
                                &                   & G4C. Does not show relevant feedback          \\ \cline{2-3} 
                                & \multirow{3}{=}{G5. Match relevant social norms - Ensure the experience is delivered in a way that users would expect, given their social and cultural context.} & G5A. Expected interaction           \\ \cline{3-3} 
                                &                   & G5B. Somewhat expected interaction           \\ \cline{3-3} 
                                &                   & G5C. Unexpected interaction          \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \hline
\multirow{21}{*}{Overtime}              & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \cline{2-3} 
                                & \multirow{3}{*}{} &           \\ \cline{3-3} 
                                &                   &           \\ \cline{3-3} 
                                &                   &           \\ \hline
\end{tabular}
    \label{tab:codes}
\end{table*}

==> tables/table-example1.tex <==
\begin{table}%[htbp]
  \centering
  \caption{Results on the summative scales, in \textit{M} (\textit{SD}), across all three GeoExplorer versions.} 
    \begin{tabular}{lcccccccccccccccccc}
    \toprule
 & \textbf{Basic} & \textbf{Plus} & \textbf{Advanced} \\
\textbf{Scale} & \textit{n} = 29 & \textit{n} = 70 & \textit{n} = 207 \\
  \midrule
    CPT Learning & 3.98 (0.53) & 4.09 (0.56) & 3.96 (0.75) \\
    Integration & 3.74 (0.46) & 4.33 (0.65) & 3.94 (0.92) \\
    Geotechnical Learning & 3.75 (0.53) & 3.97 (0.62) & 3.73 (0.80) \\
    Career & 3.07 (0.93) & 3.15 (1.02) & 3.30 (0.99) \\
    Learning & 3.82 (0.49) & 3.97 (0.57) & 3.84 (0.70) \\
    \bottomrule
    \end{tabular}
  \label{tab:general}
\end{table}

\begin{table}%[htbp]
  \centering
  \caption{Routine Correlations} 
    \begin{tabular}{lcccccccccccccccccc}
    \toprule
 & \textbf{Practice} & \textbf{Sleep} & \textbf{Exercise} & \textbf{MHC-SF} & \textbf{PSS} & \textbf{Health} & \textbf{Days Training} \\
 \midrule
\textbf{Practice} & 1\\
 \textbf{Sleep} & -.1 & 1\\
 \textbf{Exercise} & -.05 & -.08 & 1\\
 \textbf{MHC-SF} & .19 & .01 & -.05 & 1\\
 \textbf{PSS} & -.08 & .08 & -.01 & -.63*** & 1\\
 \textbf{Health} & -.01 & .07 & .01 & .27 & -.24 & 1\\
 \textbf{Days Training} & .55*** & -.06 & -.13 & .27 & -.07 & .22 & 1\\

    \bottomrule
    \end{tabular}
  \label{tab:Routine}
\end{table} 



==> tables/table-example2.tex <==
\begin{table*}%[htbp]
  \centering
  \caption{Overview of the GeoExplorer-Advanced results (\textit{n} = 207) on all individual survey items, in \textit{Mdn} (\textit{IQR}).} 
  \begin{threeparttable}
  \setlength\tabcolsep{4pt} 
    %\small
    \begin{tabular}{clcccccc}
    \toprule
   &   & \multicolumn{2}{c}{\textbf{Gender}\tnote{a}} & \multicolumn{4}{c}{\textbf{Race/Ethnicity}\tnote{b}}\\
   &   & \multicolumn{2}{c}{(\textit{n} = 191)} & \multicolumn{4}{c}{(\textit{n} = 180)}  \\
   \cmidrule(r){3-4}\cmidrule(r){5-8}
    \textbf{Item } & \textbf{Description} & F & M  & A  & L  & W & O \\
  \midrule
     \multicolumn{2}{l}{\textit{CPT Learning} ($\alpha$ = .92)}\\% & 4.01 (0.78) & 3.96 (0.71)  & 4.06 (0.64) & 4.06 (0.85) & 3.93 (0.72) & 3.76 (0.96)\\
    1 & Learn about the operation of CPT equipment.  & 4 (4 - 5)  & 4 (4 - 4)    & 4 (4 - 4.75)  & 4 (4 - 5)     & 4 (4 - 4)  & 4 (3 - 4)\\
    
    2 & Visualize subsurface stratigraphy. & 4 (4 - 4.5)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (4 - 5)    & 4 (4 - 4)    & 4 (3 - 4)     \\
 
    3 & Simulate field conditions & 4 (4 - 4.5)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (4 - 5)     & 4 (4 - 4)  & 4 (3 - 4.5)     \\

    4 & \multicolumn{1}{p{25em}}{Conduct a geotechnical site investigation using\newline{} CPT equipment.} & 4 (4 - 4.5)  & 4 (4 - 4)    & 4 (4 - 4.75)    & 4 (4 - 5)    & 4 (4 - 4)    & 4 (3 - 4.5)\\[0.35cm]

    \multicolumn{2}{l}{\textit{Integration} ($\alpha$ = .94)} \\%& 4.04 (0.85) & 3.92 (0.94) & 3.92 (0.94) & 4.14 (0.80) & 4.11 (0.72) & 3.28 (1.28)\\
    5 & \multicolumn{1}{p{25em}}{The class lectures prepared me for conducting the\newline{}CPT in the mock internship.%\newline{}(i.e., using the appropriate methods and tools to collect data about soils). 
    } & 4 (4 - 5)  & 4 (4 - 5)     & 4 (3 - 5)  & 4 (4 - 5)     & 4 (4 - 5)  & 4 (2.5 - 4)\\

    6 & \multicolumn{1}{p{25em}}{The class lectures prepared me for analyzing\newline{} the results from the CPT.} & 4 (4 - 5)  & 4 (4 - 5)     & 4 (3.25 - 5)  & 4 (4 - 5)     & 4 (4 - 4.5)  & 3 (2.5 - 4) \\
    
    7 & \multicolumn{1}{p{25em}}{The CPT Environment was a good way to put what\newline{} I learned in class into practice.} & 4 (4 - 5)  & 4 (4 - 4.5)     & 4 (3 - 5)  & 4 (4 - 5)     & 4 (4 - 5)  & 4 (3 - 4) \\[0.35cm]
    
    \multicolumn{2}{l}{\textit{Geotechnical Learning} ($\alpha$ = .90)}\\%  & 3.71 (0.84) & 3.80 (0.72) & 3.98 (0.70) & 3.76 (0.86) & 3.69 (0.74) & 3.61 (0.90) \\
    8 & Helped me understand geotechnical engineering better. & 4 (3 - 4)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (3 - 4)     & 4 (4 - 4)  & 4 (3 - 4)   \\

    9 & Made me want to learn more about geotechnical engineering. & 4 (3 - 4)  & 4 (3 - 4)     & 4 (3 - 4)  & 4 (3 - 4)    & 4 (3 - 4)      & 3 (3 - 4)     \\

    10 & Helped show me why geotechnical engineering is important. & 4 (3 - 4)  & 4 (3 - 4)     & 4 (3 - 5)  & 4 (4 - 4)     & 4 (3 - 4)  & 3.5 (3 - 4)      \\

    11 & \multicolumn{1}{p{25em}}{Was an effective way to learn about site investigation methods \newline{}that are relevant to geotechnical engineering.} & 4 (3.5 - 4.5)  & 4 (4 - 4)     & 4 (4 - 4)  & 4 (3 - 4)     & 4 (4 - 4)  & 4 (3 - 4)     \\[0.35cm]
 
    \multicolumn{2}{l}{\textit{Career} ($\alpha$ = .94)} \\% & 3.28 (1.16) & 3.34 (0.89) & 3.18 (1.08) & 3.47 (0.88) & 3.28 (1.03) & 3.30 (0.90)\\
    12 & Take more classes that focus on geotechnical engineering. & 4 (3 - 4)  & 4 (3 - 4)     & 3 (2 - 4)  & 4 (3 - 4)    & 3.5 (3 - 4)    & 4 (3 - 4)\\
    
    13 & Pursue a concentration in geotechnical engineering. & 3 (2.5 - 4)  & 3 (3 - 4)     & 3 (2 - 4)  & 3 (3 - 4)    & 3 (3 - 4)    & 3 (3 - 4)     \\

    14 & Pursue a graduate degree in geotechnical engineering. & 3 (2 - 4)  & 3 (3 - 4)    & 3 (2 - 4)    & 3 (3 - 4)    & 3 (2 - 4)    & 3 (3 - 4)     \\

    15 & Seek employment with a geotechnical engineering firm. & 3 (3 - 4)  & 3 (3 - 4)     & 3 (2 - 4)  & 4 (3 - 4)    & 3 (3 - 4)    & 3 (3 - 4)     \\%[0.5cm]
     %\multicolumn{2}{l}{\textit{Learning}\tnote{c} ($\alpha$ = .88)}  & 3.85 (0.73) & 3.86 (0.66) & 4.01 (0.64) & 3.90 (0.81) & 3.79 (0.61)  & 3.69 (0.92)\\
    \bottomrule
    \end{tabular}
    \smallskip
    \scriptsize
    \begin{tablenotes}
        \scriptsize 
        \item \textit{Gender}: F = Female; M = Male. \textit{Race/Ethnicity}: A = Asian; L = Latino/Latina or Hispanic; W = Caucasian or White; O = other race/ethnicity.
        %\item[c] Learning is a scale that combines the items of the CPT Learning and Geotechnical Engineering Learning scales minus Items 1 and 8. 
    \end{tablenotes}
  \end{threeparttable}
    \label{tab:individual}
\end{table*}

==> tables/table-games.tex <==
\definecolor{darkseagreen}{rgb}{0.56, 0.74, 0.56}
\definecolor{grannysmithapple}{rgb}{0.66, 0.89, 0.63}
\definecolor{pastelred}{rgb}{1.0, 0.41, 0.38}


\begin{table*}[!t]
\caption{Coding of the 20 selected games by the initial coders, climate/education expert, and serious games expert.}
\begin{threeparttable}
    %\small
    \centering
    \begin{tabular}{lccccccc}
        \toprule
         \textbf{Game Title}\tnote{a} & \textbf{Genre} & \textbf{Interaction Metaphor} & \textbf{Climate/Education} & \textbf{Serious Games} & \textbf{Initial}\tnote{b} & %\textbf{Consensus}\tnote{c} 
        % & \textbf{Remix}\tnote{d} \\
         & & \textbf{Coders} & \textbf{Expert} & \textbf{Expert} & \textbf{Agreement} &  & \\ 
         \hline
         \rowcolor{grannysmithapple}
         Eco-Friendly Choices* & Quiz & + & = & + & Somewhat & Balanced & No \\
         \rowcolor{pastelred}
         Monkey \& Balloons* & Quiz & - & - & - & Yes & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Albedo Pong & Pong & + & + & + & Yes & Balanced & No \\ 
         \rowcolor{pastelred}
         Save the Animals! & Pong & - & - & - & Yes & Imbalanced & No \\ 
         \rowcolor{grannysmithapple}
         Adventures of TreeGuy & Platform & + & + & + & Yes & Balanced & No\\
         \rowcolor{pastelred}
         GAMEGAMEMEGAMEGA & Platform & - & = & - & Somewhat & Imbalanced & No \\ 
         \rowcolor{grannysmithapple}
         C02 Pacman* & Maze & + & + & + & Yes & Balanced & Yes \\
         \rowcolor{pastelred}
         Jetpack Cat* & Maze & - & = & - & Somewhat & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Plants vs. Zomseas & Clicker & + & + & + & Yes & Balanced & Yes \\
         \rowcolor{pastelred}
         Defrostation* & Clicker & - & - & - & Yes & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Ice Cap Hero! & Shooter & + & + & = & Somewhat & Balanced & Yes \\
         \rowcolor{pastelred}
         Climate Change Game & Shooter & - & = & = & Somewhat & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Save the Atmosphere!\tnote{e} & Swipe & = & NA & + & Somewhat & Balanced & No \\
         \rowcolor{pastelred}
         Carbon Witch* & Swipe & - & - & - & Yes & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Carbon Crusher & Puzzle & + & + & = & Somewhat & Balanced & Yes \\
         \rowcolor{pastelred}
         Climate Change Sort Game & Puzzle & - & - & - & Yes & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Pet Earth! & Simulation & - & = & + & No & Balanced & No \\
         \rowcolor{pastelred}
         Government Simulator & Simulation & + & + & - & No & Imbalanced & No \\
         \rowcolor{grannysmithapple}
         Carbon Clicker & Storytelling & + & - & + & No & Balanced & No \\
         \rowcolor{pastelred}
         Gerald the Squirrel & Storytelling & - & - & - & Yes & Imbalanced & No \\
         \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \small
    \item[a] Many student games used their first names as title (e.g., Amanda \& George). We provided the title for their games in such instances. All the starred (*) titles are games that we named.
     \item[b] The ``Initial Agreement'' refers to how raters agreed without discussion. 
     \item[c] ``Consensus'' refers to the verdict after discussion. 
     \item[d] ``Remix'' refers to if the game was copied from another Scratch project. 
     \item[e] This game was added later because the positively rated selected game by the initial coders was judged negatively by both experts.
    %Student-designed games can be accessed as follows: \url{https://scratch.mit.edu/projects/<project ID>}. All student-designed games were accessible as of February 3, 2020. To preserve the student work, we downloaded the projects and included these as supplementary material. 
    \end{tablenotes}
    \end{threeparttable}
    \label{tab:20}
\end{table*}
